Online Versus Offline NMT Quality: An In-depth Analysis on English-German and German-English

We conduct in this work an evaluation study comparing offline and online neural machine translation architectures. Two sequence-to-sequence models: convolutional Pervasive Attention (Elbayad et al. 2018) and attention-based Transformer (Vaswani et al. 2017) are considered. We investigate, for both architectures, the impact of online decoding constraints on the translation quality through a carefully designed human evaluation on English-German and German-English language pairs, the latter being particularly sensitive to latency constraints. The evaluation results allow us to identify the strengths and shortcomings of each model when we shift to the online setup.

==> archive.tex <==
\mypar{Part-of-speech tags}
We use an off-the-shelf part-of-speech tagger~\cite{Schmid13TreeTaggeer} and count the errors per tag in \fig{postag-source}.

\laurent{For offline systems, we see the most errors for DET, NOUN and VERB, which account for the larger ratio of part-of-speech categories. More errors for PRON are observed for \engde and this trend is reinforced in online mode. 
%Interestingly, the non existing word form (ne) error mostly affects NOUN and not PROPNON. 
Concerning grammar errors (gr) they occur mostly for VERB in \deen while they are more scattered between several part-of-speech tags for \engde. We also verify that typography (ty) affects PUNCT but also NOUN for \engde (compound words + capitalization). Word order (wo) errors affect mostly VERB for \engde but also NOUN and ADV for \deen.
}


\begin{figure}
\centering
\setlength{\tabcolsep}{0pt}
\begin{tabular}{c}
    \engde \\
    \includegraphics[width=\linewidth]{srcpostags/ende} \\
    \deen \\
    \includegraphics[width=\linewidth]{srcpostags/deen} 
\end{tabular}
\caption{Count of errors per Part-of-Speech tag. Evaluated based on $\Am_1 || \Am_2$. \maha{Source side. Counts are normalized by the frequencies listed in \tab{srcpostags-count}.}}
\label{fig:postag-source}
\end{figure}

\begin{table}
\small
\setlength{\tabcolsep}{2pt}
\centering
\input{tables/srcpostags/counts}
\caption{\engde frequencies of source-side POS tags.}\label{tab:srcpostags-count}
\end{table}

\begin{table}
\tiny
\setlength{\tabcolsep}{1pt}
\centering
\begin{tabular}{cc}
    PA-offline & PA-online\\
    \input{tables/srcpostags/pa_offline} &
    \input{tables/srcpostags/pa_online} \\
    TF-offline & TF-online\\
    \input{tables/srcpostags/tf_offline} &
    \input{tables/srcpostags/tf_online}\\
\end{tabular}
\caption{\engde The values of \fig{postag-source} un-normalized.}
\end{table}




==> correlation.tex <==
\begin{table}
    \small
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{subfigure}{\linewidth}
    \centering
    \caption{PA-offline}
    \input{tables/corr/pa_offline_deen}
    \end{subfigure}\\[5pt]
    \begin{subfigure}{\linewidth}
    \centering
    \caption{PA-online}
    \input{tables/corr/pa_online_deen}
    \end{subfigure}\\[5pt]
    \begin{subfigure}{\linewidth}
    \centering
    \caption{TF-offline}
    \input{tables/corr/tf_offline_deen}
    \end{subfigure}\\[5pt]
    \begin{subfigure}{\linewidth}
    \centering
    \caption{TF-online}
    \input{tables/corr/tf_online_deen}
    \end{subfigure}
    \caption{\maha{FYI} \deen: correlation matrix (Perason's $r$). 
        We denote with $\x$, $\y$ and $\hyp$ the source, reference and hypothesis respectively. 
        BERTScore~\protect\cite{Zhang20iclr}.
        %BLEURT~\protect\cite{Sellam20acl}. 
} 
\end{table}


\begin{table}
    \small
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{subfigure}{\linewidth}
    \centering
    \caption{PA-offline}
    \input{tables/corr/pa_offline_ende}
    \end{subfigure}\\[5pt]
    \begin{subfigure}{\linewidth}
    \centering
    \caption{PA-online}
    \input{tables/corr/pa_online_ende}
    \end{subfigure}\\[5pt]
    \begin{subfigure}{\linewidth}
    \centering
    \caption{TF-offline}
    \input{tables/corr/tf_offline_ende}
    \end{subfigure}\\[5pt]
    \begin{subfigure}{\linewidth}
    \centering
    \caption{TF-online}
    \input{tables/corr/tf_online_ende}
    \end{subfigure}
    \caption{\engde} 
\end{table}




==> figures/srclength/tmp <==
xticklabels={$<13$, \bin{13}{16}, \bin{16}{18}, \bin{18}{20}, \bin{20}{23}, $\geq 23$, ($r$)},




==> issues.tex <==
\section{Inspecting short segments}
Looking at annotated samples from \deen with the highest relative count of mistranslation (mt) errors \ie $\#mt/\ly$.

\begin{table}[H]
\setlength{\tabcolsep}{2.5pt}
\input{tables/mt_length_samples}
\caption{FYI, first length bucket $\ly<14$.
5th row (ID 167):  An amazing example <ty>{\bad,}</> <mt>{\bad like}</> a nation, a state <mt>{\bad that}</> can <mt>{\bad look}</> and <mt>{\bad reach}</> <mt>{\bad rebel}</> with <mt>{\bad their}</> people.
Google translate of the source (It is an astonishing example of how a nation, a state, can seek and achieve reparation with its inhabitants.)
}
\end{table}
\begin{observations}
\item The hypothesis length would be an appropriate denominator, but, it doesn't allow for having identical bins across the 4 systems.
\item Consider length-ratio as another feature for analysis especially for online systems. It'll be highly correlated with duplication errors.
\item These 10 samples with the highest $\#mt/\ly$ are not colloquial nor oral/filler talk.
\end{observations}


==> systems.tex <==
\section{Online and offline NMT architectures}\label{sec:systems}   

In this work we train Transformer~\cite{Vaswani17nips} and Pervasive Attention~\cite{Elbayad18conll} models for the tasks of online and offline translation. We will describe in the following both systems and how they are adapted for online decoding.

\subsection{Wait-k decoding}\label{sec:waitk}
Wait-$k$ online decoding~\cite{Ma19acl,Dalvi18naacl}
 starts by reading $k$ source tokens, and  then alternates between reading and writing a single token at a time, until  the full source has been read, or the target generation has been terminated.
Formally, we denote with $z_t$ the number of source tokens read when decoding $y_t$. For a wait-$k$ decoding path we have  $z_t = \min(k+t-1, \lx).$ 

\subsection{Transformer (TF)}\label{sec:transformer}
Transformer encoder and decoder are fed a sum of token and position embeddings and
through a stack of $\Nm$ blocks, interleave multi-headed self-attention and feed-forward layers. Additionally, the decoder blocks use multi-headed attention to interact with the source states.
The key component of the transformer model \cite{Vaswani17nips} is multi-headed attention, which concatenates the outputs of multiple attention heads.
Attention aggregates encoder/decoder states from other positions in the form of a weighted sum, where the weights depend on the current state.
In the encoder-decoder attention, the decoder state $h_{t}$, used to predict $y_{t+1}$, attends to the first $z_{t+1}$ source states.
Similar to \newcite{Elbayad20arxiv}, we use unidirectional encoders.

\begin{figure}
\centering
\begin{subfigure}[b]{.25\linewidth}
\includegraphics[width=.85\textwidth]{model/offline_conv}
\caption{Offline convolution}\label{fig:offline-conv}
\end{subfigure}\hskip5pt
\begin{subfigure}[b]{.21\linewidth}
\includegraphics[width=.85\textwidth]{model/offline_pool}
\caption{Offline max-pooling}\label{fig:offline-pool}
\end{subfigure}\hskip10pt
\begin{subfigure}[b]{.25\linewidth}
\includegraphics[width=.85\textwidth]{model/online_conv}
\caption{Online convolution}\label{fig:online-conv}
\end{subfigure}\hskip5pt
\begin{subfigure}[b]{.21\linewidth}
\includegraphics[width=.85\textwidth]{model/online_pool}
\caption{Online max-pooling}\label{fig:online-pool}
\end{subfigure}
\caption{Illustration of causal two-dimensional convolutions and max-pooling for online and offline Pervasive Attention.}\label{fig:conv}
\vspace{-10pt}
\end{figure}


\subsection{Pervasive Attention (PA)}\label{sec:pervasive}
In Pervasive Attention~\cite{Elbayad18conll}, the source and target sequences are jointly encoded with a two-dimensional convolutional neural network (CNN).
For  decoding, \cite{Elbayad18conll} use causal convolutions where the filters mask future target positions (see \fig{offline-conv}). 
In a similar way, to adapt to the online translation task, we mask the filters in the source direction in order to encode the source unidirectionally (see \fig{online-conv}).
In our online version of Pervasive Attention, the CNN's ultimate features $\Hconv$ at a given position $(t,j)$ of the source-target grid encode source context up to $x_j$ and target context up to $y_t$.
In the  offline Pervasive Attention, a single representation per target position is needed to predict the next output token, which is obtained using max-pooling across the source positions (see \fig{offline-pool}). 
In the online task, we would like to make a prediction at every position where the model could be asked to write.
When predicting $y_t$ at position $(t-1,z_t)$ of the grid we max-pool the activations in $\Hconv_{t-1, \leq z_t}$ (see \fig{online-pool}). 
%\emmanuelle{[Could Figure 2 be on the same page as the PA paragraphs?]}




==> tables/agreement/deen_kappa_raw.tex <==
\begin{tabular}{lrrrrr}
\toprule
& \multicolumn{5}{c}{De$\sto$En}\\
\midrule
& \multicolumn{2}{c}{PA} & \multicolumn{2}{c}{TF} & All\\
\midrule
& Offline & Online & Offline & Online & \\ 
\midrule
Accuracy & 0.00 & 0.00 & 0.00 & 0.66 & 0.25 \\
Addition & \bad0.14 & \bad0.16 & \bad0.09 & \bad0.08 & \bad0.12 \\
Mistranslation & 0.31 & 0.20 & 0.33 & \bad0.17 & 0.26 \\
Non-existing WF & \bad0.04 & \bad0.11 & \bad0.13 & \bad0.12 & \bad0.10 \\
Omission & 0.30 & 0.30 & 0.37 & 0.33 & 0.33 \\
Overly litteral & 0.21 & \bad0.13 & \bad0.11 & \bad0.14 & \bad0.15 \\
\midrule
Fluency & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
Duplication & 0.55 & 0.36 & 0.39 & 0.52 & 0.51 \\
Grammar & \bad-0.02 & \bad0.06 & \bad0.09 & \bad0.03 & \bad0.04 \\
Typography & \bad0.12 & 0.38 & 0.21 & \bad0.17 & 0.22 \\
Unintelligible & -0.01 & 0.00 & -0.01 & -0.01 & -0.01 \\
Word order & 0.38 & 0.32 & 0.33 & 0.29 & 0.33 \\
\bottomrule
\end{tabular}


==> tables/agreement/deen_kappa_raw_bin.tex <==
\begin{tabular}{lrrrrr}
\toprule
& \multicolumn{5}{c}{De$\sto$En}\\
\midrule
& \multicolumn{2}{c}{PA} & \multicolumn{2}{c}{TF} & All\\
\midrule
& Offline & Online & Offline & Online & \\ 
\midrule
%Accuracy & 0.00 & 0.00 & 0.00 & 0.66 & 0.25 \\
%Addition & 0.19 & 0.23 & 0.20 & 0.17 & 0.21 \\
%Mistranslation & 0.57 & 0.42 & 0.62 & 0.35 & 0.51 \\
%Non-existing Word Form & 0.09 & 0.11 & 0.13 & 0.12 & 0.11 \\
%Omission & 0.35 & 0.41 & 0.49 & 0.43 & 0.43 \\
%Overly litteral & 0.25 & 0.17 & 0.15 & 0.21 & 0.20 \\
%\midrule
Average accuracy & 0.24 & 0.22 & 0.27 & 0.32 & 0.28 \\
-Accuracy & 0.29 & 0.27 & 0.32 & 0.26 & 0.29\\
\midrule
%Fluency & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%Duplication & 0.66 & 0.49 & 0.45 & 0.77 & 0.69 \\
%Grammar & -0.00 & 0.07 & 0.09 & 0.03 & 0.04 \\
%Typography & 0.15 & 0.40 & 0.24 & 0.18 & 0.24 \\
%Unintelligible & -0.01 & 0.00 & -0.01 & -0.01 & -0.01 \\
%Word order & 0.47 & 0.47 & 0.45 & 0.38 & 0.45 \\
%\midrule
Average fluency & 0.21 & 0.24 & 0.20 & 0.23 & 0.24 \\
-Fluency, Ut & 0.32 & 0.36 & 0.31 & 0.34 & 0.36 \\
\midrule
Average all & 0.23 & 0.23 & 0.23 & 0.27 & 0.26 \\
\bottomrule
\end{tabular}


==> tables/agreement/deen_kappa_span.tex <==
\begin{tabular}{lrrrrr}
\toprule
& \multicolumn{5}{c}{De$\sto$En}\\
\midrule
& \multicolumn{2}{c}{PA} & \multicolumn{2}{c}{TF} & All\\
\midrule
& Offline & Online & Offline & Online & \\ 
\midrule
Accuracy & 0.00 & 0.00 & 0.00 & 0.33 & 0.12 \\
Addition & \bad0.19 & \bad0.17 & \bad0.12 & \bad0.10 & \bad0.15 \\
Mistranslation & 0.30 & \bad0.18 & 0.30 & \bad0.13 & 0.23 \\
Non-existing WF & \bad0.04 & \bad0.11 & \bad0.14 & \bad0.12 & \bad0.10 \\
Omission & 0.29 & 0.33 & 0.41 & 0.29 & 0.33 \\
Overly literal & 0.21 & \bad0.09 & \bad0.09 & \bad0.18 & \bad0.15 \\
\midrule
Fluency & \bad0.00 & \bad0.00 & \bad0.00 & \bad0.00 & \bad0.00 \\
Duplication & 0.43 & 0.46 & 0.40 & 0.55 & 0.54 \\
Grammar & \bad-0.01 & \bad0.06 & \bad0.04 & \bad0.00 & \bad0.03 \\
Typography & \bad0.14 & 0.34 & \bad0.15 & \bad0.19 & 0.21 \\
Unintelligible & \bad-0.00 & \bad0.00 & \bad-0.00 & \bad-0.00 & \bad-0.00 \\
Word order & 0.43 & 0.33 & 0.34 & 0.28 & 0.35 \\
\bottomrule
\end{tabular}


==> tables/agreement/deen_kappa_token.tex <==
\begin{tabular}{lrrrrr}
\toprule
& \multicolumn{5}{c}{De$\sto$En}\\
\midrule
& \multicolumn{2}{c}{PA} & \multicolumn{2}{c}{TF} & All\\
\midrule
& Offline & Online & Offline & Online & \\ 
\midrule
Accuracy & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 \\
Addition & 0.28 & 0.22 & 0.27 & 0.21 & 0.24 \\
Mistranslation & 0.45 & 0.44 & 0.53 & 0.41 & 0.46 \\
Non-existing WF & \bad0.09 & \bad0.13 & \bad0.15 & \bad0.12 & \bad0.11 \\
Omission & \bad0.18 & 0.23 & 0.25 & 0.26 & 0.23 \\
Overly literal & \bad0.19 & \bad0.19 & \bad0.08 & \bad0.17 & \bad0.17 \\
\midrule
Fluency & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
Duplication & 0.47 & 0.50 & \bad0.17 & 0.55 & 0.51 \\
Grammar & \bad0.03 & \bad0.05 & \bad0.09 & \bad0.05 & \bad0.05 \\
Typography & \bad0.17 & 0.34 & \bad0.12 & \bad0.19 & 0.21 \\
Unintelligible & -0.00 & 0.00 & -0.00 & -0.00 & -0.00 \\
Word order & 0.32 & 0.42 & 0.39 & 0.28 & 0.36 \\
\bottomrule
\end{tabular}


==> tables/agreement/ende_kappa_raw.tex <==
\begin{tabular}{Hrrrrr}
\toprule
& \multicolumn{5}{c}{En$\sto$De}\\
\midrule
& \multicolumn{2}{c}{PA} & \multicolumn{2}{c}{TF} & All\\
\midrule
& Offline & Online & Offline & Online  & \\ 
\midrule
Accuracy & 1.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
Addition & \bad0.17 & 0.39 & 0.29 & 0.25 & 0.30 \\
Mistranslation & 0.21 & 0.29 & 0.25 & 0.31 & 0.27 \\
Non-existing Word Form & 0.42 & 0.53 & 0.68 & 0.67 & 0.58 \\
Omission & 0.28 & 0.35 & 0.41 & 0.43 & 0.38 \\
Overly literal & \bad0.14 & \bad0.14 & 0.22 & \bad0.08 & \bad0.15 \\
\midrule
Fluency & -0.01 & 0.00 & 0.10 & 0.00 & 0.02 \\
Duplication & \bad-0.01 & 0.24 & 0.29 & 0.48 & 0.41 \\
Grammar & 0.30 & 0.26 & 0.23 & 0.32 & 0.29 \\
Typography & 0.45 & 0.42 & 0.35 & 0.35 & 0.40 \\
Unintelligible & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
Word order & 0.40 & 0.51 & 0.57 & 0.39 & 0.47 \\
\bottomrule
\end{tabular}


==> tables/agreement/ende_kappa_raw_bin.tex <==
\begin{tabular}{Hrrrrr}
\toprule
& \multicolumn{5}{c}{En$\sto$De}\\
\midrule
& \multicolumn{2}{c}{PA} & \multicolumn{2}{c}{TF} & All\\
\midrule
& Offline & Online & Offline & Online  & \\ 
\midrule
%Accuracy & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%Addition & 0.17 & 0.40 & 0.32 & 0.36 & 0.35 \\
%Mistranslation & 0.34 & 0.38 & 0.34 & 0.41 & 0.37 \\
%Non-existing Word Form & 0.42 & 0.54 & 0.70 & 0.69 & 0.59 \\
%Omission & 0.35 & 0.48 & 0.47 & 0.54 & 0.47 \\
%Overly litteral & 0.16 & 0.18 & 0.24 & 0.10 & 0.17 \\
%\midrule
Average Accuracy & 0.24 & 0.33 & 0.34 & 0.35 & 0.33 \\
-Accuracy & 0.29 & 0.40 & 0.41 & 0.42 & 0.39 \\
\midrule
%Fluency & -0.01 & 0.00 & 0.10 & 0.00 & 0.02 \\
%Duplication & -0.01 & 0.24 & 0.29 & 0.55 & 0.45 \\
%Grammar & 0.44 & 0.38 & 0.35 & 0.45 & 0.42 \\
%Typography & 0.50 & 0.44 & 0.37 & 0.36 & 0.42 \\
%Unintelligible & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%Word order & 0.42 & 0.56 & 0.57 & 0.43 & 0.50 \\
%\midrule
Average fluency & 0.22 & 0.27 & 0.28 & 0.30 & 0.30 \\
-Fluency, Ut  & 0.34 & 0.41 & 0.39 & 0.45 & 0.45 \\ 
\midrule
Average All & 0.23 & 0.30 & 0.31 & 0.32 & 0.31 \\
\bottomrule
\end{tabular}




==> tables/agreement/ende_kappa_span.tex <==
\begin{tabular}{Hrrrrr}
\toprule
& \multicolumn{5}{c}{En$\sto$De}\\
\midrule
& \multicolumn{2}{c}{PA} & \multicolumn{2}{c}{TF} & All\\
\midrule
& Offline & Online & Offline & Online  & \\ 
\midrule
Accuracy & 1.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
Addition & \bad0.17 & 0.34 & 0.31 & 0.23 & 0.28 \\
Mistranslation & 0.23 & 0.25 & 0.24 & 0.31 & 0.26 \\
Non-existing WF & 0.39 & 0.49 & 0.65 & 0.59 & 0.53 \\
Omission & 0.25 & 0.30 & 0.37 & 0.43 & 0.35 \\
Overly literal & \bad0.13 & \bad0.13 & \bad0.16 & \bad0.08 & \bad0.13 \\
\midrule
Fluency & \bad-0.01 & \bad0.00 & \bad0.05 & \bad0.00 & \bad0.01 \\
Duplication & \bad-0.01 & \bad0.18 & 0.22 & 0.41 & 0.34 \\
Grammar & 0.29 & 0.26 & 0.26 & 0.30 & 0.29 \\
Typography & 0.47 & 0.43 & 0.37 & 0.36 & 0.41 \\
Unintelligible & \bad0.00 & \bad0.00 & \bad0.00 & \bad0.00 & \bad0.00 \\
Word order & 0.41 & 0.47 & 0.55 & 0.35 & 0.44 \\
\bottomrule
\end{tabular}


==> tables/agreement/ende_kappa_token.tex <==
\begin{tabular}{Hrrrrr}
\toprule
& \multicolumn{5}{c}{En$\sto$De}\\
\midrule
& \multicolumn{2}{c}{PA} & \multicolumn{2}{c}{TF} & All\\
\midrule
& Offline & Online & Offline & Online  & \\ 
\midrule
Accuracy & 1.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
Addition & \bad0.12 & 0.39 & \bad0.15 & 0.29 & 0.28 \\
Mistranslation & 0.39 & 0.43 & 0.37 & 0.43 & 0.41 \\
Non-existing WF & 0.44 & 0.56 & 0.66 & 0.66 & 0.59 \\
Omission & 0.31 & 0.26 & 0.32 & 0.40 & 0.33 \\
Overly literal & 0.21 & 0.27 & 0.22 & 0.15 & 0.22 \\
\midrule
Fluency & \bad-0.00 & \bad0.00 & \bad0.05 & \bad0.00 & \bad0.01 \\
Duplication & \bad-0.00 & \bad0.14 & 0.20 & 0.45 & 0.36 \\
Grammar & 0.37 & 0.37 & 0.29 & 0.43 & 0.38 \\
Typography & 0.41 & 0.45 & 0.39 & 0.35 & 0.40 \\
Unintelligible & \bad0.00 & \bad0.00 & \bad0.00 & \bad0.00 & \bad0.00 \\
Word order & 0.35 & 0.41 & 0.39 & 0.30 & 0.36 \\
\bottomrule
\end{tabular}


==> tables/agreement/kappa_token_all.tex <==
\begin{tabular}{lrr|rr|r|rr|rr|r}
\toprule
& \multicolumn{5}{c}{{\deen}} & \multicolumn{5}{c}{{\engde}}\\ 
\hline 
& \multicolumn{2}{c|}{PA} & \multicolumn{2}{c|}{TF}  & all & \multicolumn{2}{c|}{PA} & \multicolumn{2}{c|}{TF} & all \\ 
\midrule
& Offline & Online  & Offline & Online  &    & Offline & Online & {Offline} & {Online}  & \\ 
%\makecell[l]{Kappa \\on error type} 
$\kappa$ & 0.41 &  0.40 & 0.44 & 0.41 & 0.41  & 0.43 & 0.45 & 0.43 & 0.45 & 0.44 \\
%\makecell[l]{Kappa \\on absence/presence \\of errors} 
Binary $\kappa$ & 0.58 & 0.58 & 0.61 & 0.59 & 0.59 & 0.64 & 0.66 & 0.64 & 0.69 & 0.66 \\ 
\bottomrule
\end{tabular}


==> tables/agreement/per_length.tex <==
\begin{tabular}{rrrrrrr}
\toprule
\cmidrule[0.5pt]{2-6}
$\lhyp$ & $<12$ & \bin{12}{16} & \bin{16}{20} & \bin{20}{24} & $\geq24$  & \\ 
\midrule
\engde ($\kappa$) & 0.439 & 0.484 & 0.379 & 0.412 & 0.340 & 0.404 \\
\midrule
\deen ($\kappa$) & 0.428 & 0.368 & 0.340 & 0.307 & 0.272 & 0.332 \\
\bottomrule
\end{tabular}


==> tables/agreement/rosenberg.tex <==
\begin{tabular}{lrrrrr}
\toprule
& \multicolumn{2}{c}{PA} & \multicolumn{2}{c}{TF} & All\\
\midrule
& Offline & Online & Offline & Online & \\ 
\midrule
De$\sto$En & 0.15 & 0.14 & 0.15 & 0.11 & 0.14\\
En$\sto$De & 0.16 & 0.16 & 0.18 & 0.14 & 0.16\\
\bottomrule
\end{tabular}


==> tables/agreement/token_agreement.tex <==
\begin{tabular}{lrrr}
\toprule
           & Binary & Jaccard & MASI \\
\midrule
De$\sto$En & 0.401 & 0.411 & 0.407 \\
En$\sto$De & 0.446 & 0.454 & 0.451 \\
\bottomrule
\end{tabular}


%ende- Kappa(binary) = 0.446
%ende- Alpha(binary) = 0.445
%ende- Kappa(jaccard) = 0.454
%ende- Alpha(jaccard) = 0.452
%ende- Kappa(masi) = 0.451
%ende- Alpha(masi) = 0.450


%deen- Kappa(binary) = 0.401
%deen- Alpha(binary) = 0.401
%deen- Kappa(jaccard) = 0.411
%deen- Alpha(jaccard) = 0.409
%deen- Kappa(masi) = 0.407
%deen- Alpha(masi) = 0.406


==> tables/archive/confusion.tex <==
\begin{subfigure}[b]{.3\linewidth}
\begin{tabular}{r|rrrr}
& 0 & 1 & 2 & 3 \\
\hline
0 & 640 &  34 &   0 &   1 \\
1 &  73 &  32 &   6 &   0 \\
2 &   7 &   5 &   1 &   0 \\
3 &   1 &   0 &   0 &   0 \\
\hline
\end{tabular}
\caption{En$\sto$De - \textbf{Addition}}
\end{subfigure}
\begin{subfigure}[b]{.5\linewidth}
\begin{tabular}{r|rrrrrrrrr}
& 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
\hline
0 & 556 & 123 &  39 &  23 &   6 &   1 &   0 &   0 &   2 \\
1 &   9 &  12 &   9 &   8 &   7 &   2 &   1 &   0 &   1 \\
2 &   0 &   0 &   1 &   0 &   0 &   0 &   0 &   0 &   0 \\
3 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\
4 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\
5 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\
6 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\
7 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\
8 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\
\hline
\end{tabular}
\caption{De$\sto$En - \textbf{Addition}}
\end{subfigure}\\
\begin{subfigure}[b]{.4\linewidth}
\begin{tabular}{r|rrrrr}
& 0 & 1 & 2 & 3 & 4 \\
\hline
0 & 317 & 158 &  47 &  13 &   1 \\
1 &  38 & 113 &  46 &   9 &   2 \\
2 &   4 &  15 &  15 &  10 &   0 \\
3 &   0 &   4 &   3 &   5 &   0 \\
4 &   0 &   0 &   0 &   0 &   0 \\
\hline
\end{tabular}
\caption{En$\sto$De- \textbf{Mistranslation}}
\end{subfigure}
\begin{subfigure}[b]{.45\linewidth}
\begin{tabular}{r|rrrrrrr}
& 0 & 1 & 2 & 3 & 4 & 5 & 6 \\ 
\hline
0 & 162 &  67 &  26 &  11 &   6 &   0 &   0 \\ 
1 &  47 & 121 &  79 &  28 &   8 &   5 &   0 \\ 
2 &  10 &  42 &  56 &  29 &  17 &   2 &   1 \\ 
3 &   1 &  14 &  13 &  11 &  10 &   5 &   2 \\ 
4 &   0 &   1 &   4 &   7 &   6 &   0 &   1 \\ 
5 &   0 &   0 &   1 &   2 &   2 &   2 &   0 \\ 
6 &   0 &   0 &   0 &   0 &   0 &   1 &   0 \\ 
\hline
\end{tabular}
\caption{De$\sto$En - \textbf{Mistranslation}}
\end{subfigure}\\
\vspace{10pt}
\begin{subfigure}[b]{.4\linewidth}
\begin{tabular}{r|rrrrr}
& 0 & 1 & 2 & 3 & 4 \\
\hline
0 & 730 &   7 &   0 &   0 &   0 \\
1 &  40 &  17 &   0 &   0 &   0 \\
2 &   1 &   3 &   0 &   0 &   1 \\
3 &   0 &   0 &   0 &   1 &   0 \\
4 &   0 &   0 &   0 &   0 &   0 \\
\hline
\end{tabular}
\caption{En$\sto$De - \textbf{Duplication}}
\end{subfigure}
\begin{subfigure}[b]{.4\linewidth}
\begin{tabular}{r|rrrrrr}
& 0 & 1 & 2 & 3 & 4 & 5 \\ 
\hline
0 & 708 &  16 &  10 &   0 &   0 &   0 \\ 
1 &  13 &  25 &  14 &   3 &   5 &   2 \\ 
2 &   0 &   1 &   0 &   0 &   0 &   0 \\ 
3 &   1 &   0 &   0 &   1 &   0 &   0 \\ 
4 &   0 &   0 &   0 &   1 &   0 &   0 \\ 
5 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
\hline
\end{tabular}
\caption{De$\sto$En - \textbf{Duplication}}
\end{subfigure}\\
\begin{subfigure}[b]{.4\linewidth}
\begin{tabular}{r|rrrrr}
& 0 & 1 & 2 & 3 & 4 \\ 
\hline
0 & 551 &  38 &   0 &   0 &   0 \\ 
1 &  96 &  68 &   8 &   0 &   0 \\ 
2 &  13 &  17 &   2 &   0 &   0 \\ 
3 &   0 &   3 &   2 &   1 &   0 \\ 
4 &   0 &   0 &   1 &   0 &   0 \\ 
\hline
\end{tabular}
\caption{En$\sto$De - \textbf{Omission}}
\end{subfigure}
\begin{subfigure}[b]{.4\linewidth}
\begin{tabular}{r|rrrrrr}
& 0 & 1 & 2 & 3 & 4 & 5 \\
\hline
0 & 564 &  93 &  17 &   2 &   3 &   1 \\
1 &  33 &  54 &  19 &   4 &   2 &   0 \\
2 &   0 &   4 &   1 &   1 &   0 &   0 \\
3 &   1 &   0 &   0 &   0 &   0 &   0 \\
4 &   0 &   1 &   0 &   0 &   0 &   0 \\
5 &   0 &   0 &   0 &   0 &   0 &   0 \\
\hline
\end{tabular}
\caption{De$\sto$En - \textbf{Omission}}
\end{subfigure}



==> tables/archive/deen_errors_raw_pt.tex <==
\begin{tabular}{lrrr|rrr|}
\toprule
& \multicolumn{6}{c|}{De$\sto$En}\\
\midrule
& \multicolumn{3}{c|}{PA} & \multicolumn{3}{c|}{TF}\\
\midrule
System & Offline & Online & $\Delta\%$ & Offline & Online & $\Delta\%$\\
\midrule
Accuracy &   0.06 &   0.03 & -50 &   0.06 &   0.09 &  50\\
Addition &  2.25 &  4.23 & 88 &  2.81 &  4.74 & 68 \\
Mistranslation & 12.82 & 17.38 & 36 & 13.53 & 16.93 & 25\\
Non-existing WF &   0.77 &   0.50 & -35 &   0.41 &   0.47 &  14 \\
Omission &  1.98 &  3.35 & 69 &  2.84 &  3.76 & 32\\
Overly litteral &  2.31 &  2.81 & 22 &  1.54 &  2.40 & 56 \\
\midrule
Total accuracy & 20.19 & 28.30 & 40 & 21.20 & 28.39 & 34 \\
\midrule
Fluency &  0.50 &  0.59 & 18 &  0.41 &  0.59 & 43 \\
Duplication &   0.33 &   0.95 & 191 &   0.65 &   4.26 & 555 \\
Grammar &  1.69 &  1.92 & 14 &  1.07 &  1.01 & -6 \\
Typography &  1.21 &  1.24 &  2 &  0.98 &  1.75 & 79 \\
Unintelligible &  0.06 &  0.09 & 50 &  0.06 &  0.06 &  0\\
Word order &  1.92 &  3.11 & 62 &  1.95 &  2.31 & 18\\
\midrule
Total fluency &  5.71 &  7.90 & 38 &  5.12 &  9.98 & 95\\
\midrule
Total & 25.90 & 36.20 & 40 & 26.32 & 38.37 & 46 \\
%Hyplength & 3400 & 3460 &    1.76 & 3327 & 3610 &    8.51 \\
%Reflength & 3378 & 3378 &    0.00 & 3378 & 3378 &    0.00 \\
\bottomrule
\end{tabular}


==> tables/archive/deen_errors_span.tex <==
\begin{tabular}{lrrr|rrr}
\toprule
& \multicolumn{6}{c}{De$\sto$En}\\
\midrule
& \multicolumn{3}{c|}{PA} & \multicolumn{3}{c}{TF}\\
\midrule
System & Offline & Online & $\Delta\%$ & Offline & Online & $\Delta\%$\\
\midrule
Accuracy &   4 &   2 & -50 &   7 &   7 &   0 \\
Addition & 130 & 248 & \bad91 & 150 & 269 &  \bad79 \\
Mistranslation & 738 & 961 &  30 & 700 & 958 &  37 \\
Non-existing WF &  44 &  29 & \good-34 &  25 &  32 &  28 \\
Omission &  68 &  95 &  40 &  82 & 117 &  43 \\
Overly litteral & 151 & 182 &  21 & 103 & 155 &  \bad50 \\
\midrule
Total accuracy &  984 & 1335 &   36 &  964 & 1383 &   43 \\
\midrule
Fluency & 49 & 62 & 27 & 40 & 66 & \bad65 \\
Duplication &  16 &  53 & \bad231 &  42 & 231 & \bad450 \\
Grammar & 123 & 147 &  20 &  79 &  73 &  \good-8 \\
Typography &  70 &  63 & \good-10 &  58 & 105 &  \bad81 \\
Unintelligible &  11 &  29 & \bad164 &  12 &  17 &  42 \\
Word order & 117 & 185 &  \bad58 & 114 & 140 &  23 \\
\midrule
Total fluency & 537 & 721 &  34 & 448 & 787 &  \bad76 \\
\midrule
Total & 1521 & 2056 &   35 & 1412 & 2170 &   \bad54 \\
\bottomrule
\end{tabular}


==> tables/archive/deen_postags_addition.tex <==
\begin{tabular}{|Hlll|lll}
\toprule
& \multicolumn{6}{c}{De$\sto$En}\\
\midrule
& \multicolumn{6}{c}{Addition}\\
\midrule
& \multicolumn{3}{c|}{PA} & \multicolumn{3}{c}{TF}\\
\midrule
Tag & F& O& $\Delta\%$ & F& O& $\Delta\%$\\
\midrule
PP &   7 &  27 & \bad286 &   6 &  21 & \bad250 \\
MD &   1 &   3 & 200 &   2 &   5 & 150 \\
\rowcolor{gray!50}RB &  16 &  14 & -12 &  14 &  18 &  29 \\
\rowcolor{gray!50}VB &  10 &  21 & \bad110 &   7 &  19 & 171 \\
\rowcolor{gray!50}NN &  11 &  27 & \bad145 &  13 &  24 &  \bad85 \\
\rowcolor{gray!50}IN &  11 &  28 & \bad155 &  19 &  32 &  \bad68 \\
\rowcolor{gray!50}DT &  11 &  21 &  \bad91 &   8 &  21 & \bad162 \\
, &   2 &   6 &   \bad200 &   4 &  13 & \bad225 \\
CD &   0 &   1 & $\infty$ &   0 &   1 & $\infty$ \\
NNS &   6 &   9 &  50 &  10 &   7 & \good-30 \\
WDT &   3 &   2 & -33 &   1 &   2 & 100 \\
VBP &   5 &  14 & \bad180 &   6 &  22 & \bad267 \\
RP &   1 &   0 & -100 &   1 &   2 & 100 \\
\rowcolor{gray!50}VBZ &  12 &  10 & -17 &   8 &   7 & -12 \\
SENT &   3 &   2 & -33 &   2 &   2 &   0 \\
VBD &   5 &   3 & -40 &  10 &   8 & -20 \\
TO &   6 &  20 & \bad233 &  11 &  14 &  27 \\
CC &   3 &   7 & \bad133 &   3 &   5 &  67 \\
JJ &   4 &  11 & \bad175 &  12 &  12 &   0 \\
VBG &  6 & 10 & 67 &  7 & 12 & 71 \\
NP &   2 &   4 & \bad100 &   0 &   6 & $\bad\infty$\\
PP\$ &   0 &   1 & $\infty$&   0 &   0 &  0\\
%RBR &   1 &   0 & -100 &   0 &   0 & 0 \\
VBN &   0 &   3 & $\bad\infty$&   2 &  11 & 450 \\
%POS &   0 &   1 & $\infty$ &   0 &   0 & 0 \\
%WP &   2 &   1 & -50 &   1 &   2 & 100 \\
%WRB &   2 &   1 & -50 &   2 &   1 & -50 \\
%PDT &   0 &   0 & 0 &   0 &   0 & 0 \\
%RBS &   0 &   0 & 0 &   0 &   0 & 0 \\
%`` &   0 &   0 & 0 &   0 &   0 & 0 \\
%'' &   0 &   0 & 0 &   1 &   0 & -100 \\
%JJR &   0 &   0 & 0 &   0 &   0 & 0 \\
%EX &   0 &   1 & $\infty$ &   0 &   1 & $\infty$ \\
%: &   0 &   0 & 0 &   0 &   1 & $\infty$ \\
%JJS &   0 &   0 & 0 &   0 &   0 & 0 \\
%NPS &   0 &   0 & 0 &   0 &   0 & 0 \\
%UH &   0 &   0 & 0 &   0 &   0 & 0 \\
%WP\$ &   0 &   0 & 0 &   0 &   0 & 0 \\
\bottomrule
\end{tabular}


==> tables/archive/deen_postags_duplication.tex <==
\begin{tabular}{|Hlll|lll}
\toprule
& \multicolumn{6}{c}{De$\sto$En}\\
\midrule
& \multicolumn{6}{c}{Duplication}\\
\midrule
& \multicolumn{3}{c|}{PA} & \multicolumn{3}{c}{TF}\\
\midrule
Tag & F& O& $\Delta\%$ & F& O& $\Delta\%$\\
\midrule
\rowcolor{gray!50}PP &   3 &   8 & 167 &   7 &  21 & 200 \\
MD &   0 &   2 & $\infty$ &   0 &   2 & $\infty$ \\
\rowcolor{gray!50}RB &    0 &    2 &  $\infty$ &    1 &   16 & 1500 \\
VB &   0 &   7 & $\infty$ &   4 &   9 & 125 \\
\rowcolor{gray!50}NN &    3 &    5 &   67 &    2 &   31 & 1450 \\
\rowcolor{gray!50}IN &   1 &   5 & 400 &   2 &  12 & 500 \\
\rowcolor{gray!50}DT &   0 &   2 & $\infty$ &   3 &  19 & 533 \\
\rowcolor{gray!50}, &    1 &    1 &    0 &    2 &   28 & 1300 \\
CD &   0 &   0 & 0 &   0 &   6 & $\infty$ \\
\rowcolor{gray!50}NNS &   0 &   3 & $\infty$ &   1 &  10 & 900 \\
WDT &   0 &   0 & 0 &   0 &   0 & 0 \\
\rowcolor{gray!50}VBP &   2 &   3 &  50 &   4 &  15 & 275 \\
RP &   0 &   0 & 0 &   0 &   0 & 0 \\
VBZ &   1 &   3 & 200 &   2 &   1 & -50 \\
SENT &   0 &   1 & $\infty$ &   1 &   8 & 700 \\
VBD &   1 &   0 & -100 &   1 &   8 & 700 \\
TO &   0 &   2 & $\infty$ &   2 &   4 & 100 \\
CC &   2 &   2 &   0 &   3 &   7 & 133 \\
\rowcolor{gray!50}JJ &    0 &    5 &  $\infty$ &    1 &   13 & 1200 \\
VBG &   0 &   0 & 0 &   1 &   2 & 100 \\
NP &   0 &   0 & 0 &   1 &   6 & 500 \\
PP\$ &   0 &   1 & $\infty$ &   0 &   1 & $\infty$ \\
%RBR &   1 &   0 & -100 &   0 &   0 & 0 \\
VBN &  1 &  1 &  0 &  2 &  4 & 100 \\
%POS &   0 &   0 & 0 &   0 &   0 & 0 \\
%WP &   0 &   0 & 0 &   0 &   3 & $\infty$ \\
%WRB &   0 &   0 & 0 &   1 &   2 & 100 \\
%PDT &   0 &   0 & 0 &   0 &   0 & 0 \\
%RBS &   0 &   0 & 0 &   0 &   1 & $\infty$ \\
%`` &   0 &   0 & 0 &   1 &   0 & -100 \\
%'' &   0 &   0 & 0 &   0 &   1 & $\infty$ \\
%JJR &   0 &   0 & 0 &   0 &   0 & 0 \\
%EX &   0 &   0 & 0 &   0 &   0 & 0 \\
%: &   0 &   0 & 0 &   0 &   1 & $\infty$ \\
%JJS &   0 &   0 & 0 &   0 &   0 & 0 \\
%NPS &   0 &   0 & 0 &   0 &   0 & 0 \\
%UH &   0 &   0 & 0 &   0 &   0 & 0 \\
%WP\$ &   0 &   0 & 0 &   0 &   0 & 0 \\
\bottomrule
\end{tabular}


==> tables/archive/deen_postags_mistranslation.tex <==
\begin{tabular}{rrlll|lll}
\toprule
& & \multicolumn{6}{c}{De$\sto$En}\\
\midrule
& & \multicolumn{6}{c}{Mistranslation}\\
\midrule
& & \multicolumn{3}{c|}{PA} & \multicolumn{3}{c}{TF}\\
\midrule
& Tag & F& O& $\Delta\%$ & F& O& $\Delta\%$\\
\midrule
\rowcolor{gray!50}
Personal pronoun & PP &  33 &  71 & \bad115 &  38 &  74 &  \bad95 \\ 
Modal & MD &   4 &  16 & \bad300 &   9 &  26 & \bad189 \\ 
Adverb & RB & 40 & 52 & 30 & 41 & 48 & 17 \\ 
\rowcolor{gray!50}
Verb, base form & VB & 38 & 66 & 74 & 35 & 59 & 69 \\ 
\rowcolor{gray!50}
Noun, singular & NN & 124 & 135 &   9 & 101 & 135 &  34 \\ 
\rowcolor{gray!50}
Preposition/subord. conj. & IN & 70 & 89 & 27 & 60 & 77 & 28 \\ 
\rowcolor{gray!50}
Determiner & DT & 81 & 83 &  2 & 67 & 80 & 19 \\ 
& , & 22 & 29 & 32 & 32 & 34 &  6 \\ 
Cardinal number & CD &   6 &   6 &   \good0 &   9 &   8 & \good-11 \\ 
Noun, plural & NNS & 32 & 43 & 34 & 37 & 46 & 24 \\ 
Wh-determiner & WDT &   7 &   7 &   \good0 &   4 &  10 & \bad150 \\ 
Verb, pres non-3rd p. & VBP &  25 &  50 & \bad100 &  25 &  52 & \bad108 \\ 
Particle & RP &   9 &   6 & \good-33 &   5 &  10 & \bad100 \\ 
Verb, 3rd p. sing & VBZ & 36 & 38 &  6 & 29 & 33 & 14 \\ 
End punctuation	 & SENT &  8 & 11 & 38 &  9 & 15 & 67 \\ 
Verb, past & VBD & 22 & 26 & 18 & 27 & 31 & 15 \\ 
To & TO &  20 &  46 & \bad130 &  24 &  34 &  42 \\ 
Coordinating conjunction & CC & 18 & 18 &  \good0 & 12 & 17 & 42 \\ 
\rowcolor{gray!50}
Adjective & JJ & 55 & 60 &  9 & 52 & 49 & \good-6 \\ 
Verb, gerund/participle & VBG & 18 & 30 & 67 & 21 & 30 & 43 \\ 
Proper noun, singular& NP &  19 &  17 & \good-11 &  17 &  20 &  18 \\ 
Possessive pronoun	& PP\$ &  10 &   8 & \good-20 &   5 &   2 & \good-60 \\ 
%Adverb, comparative	 & RBR &  2 &  4 & 100 &  1 &  2 & 100 \\ 
Verb be, past participle & VBN & 17 & 27 & 59 & 21 & 36 & 71 \\ 
%Possessive ending & POS &   1 &   3 & 200 &   1 &   1 &   0 \\ 
%Wh-pronoun	& WP &   8 &   7 & \good-12 &   5 &   9 &  80 \\ 
%Wh-abverb & WRB &  2 &  3 & 50 &  3 &  5 & 67 \\ 
%Predeterminer & PDT &   2 &   2 &   0 &   0 &   0 & 0 \\ 
%Adverb, superlative	 & RBS &   0 &   0 & 0 &   0 &   1 & $\infty$ \\ 
%& `` &   4 &   3 & -25 &   5 &   3 & -40 \\ 
%& '' &   1 &   1 &   0 &   1 &   3 & 200 \\ 
%Adjective, comparative & JJR &   2 &   2 &   0 &   1 &   5 & 400 \\ 
%Existential there	& EX &   1 &   0 & -100 &   2 &   1 & -50 \\ 
%& : &  1 &  1 &  0 &  1 &  2 & 100 \\ 
%Adjective, superlative	& JJS &   0 &   1 & $\infty$ &   0 &   0 & 0 \\ 
%Proper noun, plural	& NPS &   0 &   0 & 0 &   0 &   0 & 0 \\ 
%Interjection & UH &   0 &   0 & 0 &   0 &   0 & 0 \\ 
%Possessive wh-pronoun & WP\$ &   0 &   0 & 0 &   0 &   0 & 0 \\ 
\bottomrule
\end{tabular}


==> tables/archive/deen_postags_ol.tex <==
\begin{tabular}{|Hlll|lll}
\toprule
& \multicolumn{6}{c}{De$\sto$En}\\
\midrule
& \multicolumn{6}{c}{Overly literal}\\
\midrule
& \multicolumn{3}{c|}{PA} & \multicolumn{3}{c}{TF}\\
\midrule
Tag & F& O& $\Delta\%$ & F& O& $\Delta\%$\\
\midrule
\rowcolor{gray!50}PP &   9 &  15 &  67 &   6 &  13 & \bad117 \\
MD &   3 &   1 & -67 &   3 &   1 & -67 \\
\rowcolor{gray!50}RB & 10 & 10 & 0 & 6 & 6 & 0 \\
\rowcolor{gray!50}VB &  10 &   7 & \good-30 &   6 &   9 &  50 \\
\rowcolor{gray!50}NN & 20 & 25 & 25 & 15 & 25 & 67 \\
\rowcolor{gray!50}IN &  19 &  23 &  21 &  16 &  14 & \good-12 \\
\rowcolor{gray!50}DT & 13 & 18 & 38 &  8 & 15 & 88 \\
\rowcolor{gray!50}, &   8 &   6 & \good-25 &   3 &   6 & \bad100 \\
CD &   0 &   0 & 0 &   0 &   2 & $\infty$ \\
\rowcolor{gray!50}NNS &  6 &  9 & 50 &  4 &  7 & 75 \\
WDT &   1 &   1 &   0 &   0 &   1 & $\infty$ \\
\rowcolor{gray!50}VBP &   5 &   9 &  80 &   3 &   8 & \bad167 \\
RP &   3 &   3 &   0 &   2 &   5 & \bad150 \\
VBZ &   5 &   1 & \bad-80 &   1 &   3 & 200 \\
SENT &   0 &   3 & $\infty$ &   1 &   1 &   0 \\
\rowcolor{gray!50}VBD &  6 &  8 & 33 &  5 &  7 & 40 \\
\rowcolor{gray!50}TO &   7 &  10 &  43 &   5 &   4 & -20 \\
CC &  1 &  2 & 100 &  1 &  2 & 100 \\
\rowcolor{gray!50}JJ & 10 & 15 & 50 &  8 &  9 & 12 \\
VBG &  4 &  5 & 25 &  4 &  4 &  0 \\
NP &   1 &   0 & -100 &   0 &   1 & $\infty$ \\
PP\$ &   2 &   1 & -50 &   1 &   0 & -100 \\
%RBR &   0 &   1 & $\infty$ &   0 &   1 & $\infty$ \\
VBN &  4 &  4 &  0 &  4 &  5 & 25 \\
%POS &   0 &   0 & 0 &   0 &   1 & $\infty$ \\
%WP &   2 &   1 & -50 &   0 &   1 & $\infty$ \\
%WRB &   0 &   0 & 0 &   0 &   0 & 0 \\
%PDT &   1 &   1 &   0 &   1 &   0 & -100 \\
%RBS &   0 &   0 & 0 &   0 &   1 & $\infty$ \\
%`` &   0 &   1 & $\infty$ &   0 &   1 & $\infty$ \\
%'' &   0 &   0 & 0 &   0 &   0 & 0 \\
%JJR &   1 &   1 &   0 &   0 &   1 & $\infty$ \\
%EX &   0 &   0 & 0 &   0 &   1 & $\infty$ \\
%: &   0 &   0 & 0 &   0 &   0 & 0 \\
%JJS &   0 &   1 & $\infty$ &   0 &   0 & 0 \\
%NPS &   0 &   0 & 0 &   0 &   0 & 0 \\
%UH &   0 &   0 & 0 &   0 &   0 & 0 \\
%WP\$ &   0 &   0 & 0 &   0 &   0 & 0 \\
\bottomrule
\end{tabular}


==> tables/archive/deen_postags_wo.tex <==
\begin{tabular}{|Hlll|lll}
\toprule
& \multicolumn{6}{c}{De$\sto$En}\\
\midrule
& \multicolumn{6}{c}{Word order}\\
\midrule
& \multicolumn{3}{c|}{PA} & \multicolumn{3}{c}{TF}\\
\midrule
Tag & F& O& $\Delta\%$ & F& O& $\Delta\%$\\
\midrule
\rowcolor{gray!50}PP &   7 &  12 &  71 &  13 &   7 & \good-46 \\
MD &  2 &  4 & 100 &  2 &  4 & 100 \\
\rowcolor{gray!50}RB & 10 & 16 & 60 & 14 & 15 &  7 \\
\rowcolor{gray!50}VB &   6 &  13 & \bad117 &   5 &   5 &   0 \\
\rowcolor{gray!50}NN & 27 & 32 & 19 & 11 & 22 & 100 \\
\rowcolor{gray!50}IN &  17 &  13 & \good-24 &   5 &   8 &  60 \\
\rowcolor{gray!50}DT & 12 & 11 & \good-8 &  4 &  4 &  0 \\
\rowcolor{gray!50}, &   4 &  10 & \bad150 &   6 &   9 &  50 \\
CD &   2 &   1 & -50 &   1 &   1 &   0 \\
NNS &   4 &   7 &  75 &   3 &   8 & \bad167 \\
WDT &   0 &   0 & 0 &   0 &   2 & $\infty$ \\
\rowcolor{gray!50}VBP &   4 &   9 & \bad125 &   8 &   9 &  12 \\
RP &   0 &   0 & 0 &   1 &   0 & -100 \\
\rowcolor{gray!50}VBZ &   3 &   8 & \bad167 &   6 &   5 & -17 \\
SENT &   0 &   2 & $\infty$ &   1 &   3 & 200 \\
\rowcolor{gray!50}VBD &   2 &   9 & \bad350 &   9 &   9 &   0 \\
\rowcolor{gray!50}TO &   1 &   8 & \bad700 &   2 &   3 &  50 \\
CC &   0 &   5 & $\infty$ &   3 &   3 &   0 \\
\rowcolor{gray!50}JJ &  7 & 10 & 43 &  7 & 11 & 57 \\
VBG &   1 &   2 & 100 &   3 &   1 & -67 \\
NP &   1 &   5 & 400 &   3 &   2 & -33 \\
PP\$ &   0 &   1 & $\infty$ &   0 &   0 & 0 \\
%RBR &   0 &   0 & 0 &   1 &   0 & -100 \\
VBN &  3 &  3 &  0 &  3 &  6 & 100 \\
%POS &   0 &   1 & $\infty$ &   0 &   0 & 0 \\
%WP &   1 &   0 & -100 &   0 &   0 & 0 \\
%WRB &   0 &   0 & 0 &   0 &   0 & 0 \\
%PDT &   0 &   0 & 0 &   0 &   0 & 0 \\
%RBS &   0 &   0 & 0 &   0 &   0 & 0 \\
%`` &   0 &   0 & 0 &   0 &   0 & 0 \\
%'' &   1 &   0 & -100 &   2 &   1 & -50 \\
%JJR &   2 &   2 &   0 &   0 &   2 & $\infty$ \\
%EX &   0 &   1 & $\infty$ &   1 &   0 & -100 \\
%: &   0 &   0 & 0 &   0 &   0 & 0 \\
%JJS &   0 &   0 & 0 &   0 &   0 & 0 \\
%NPS &   0 &   0 & 0 &   0 &   0 & 0 \\
%UH &   0 &   0 & 0 &   0 &   0 & 0 \\
%WP\$ &   0 &   0 & 0 &   0 &   0 & 0 \\
\bottomrule
\end{tabular}


==> tables/archive/diff_pa_offline_deen.tex <==
\begin{tabular}{lrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | PA-offline}\\
\midrule
    Difficulty & \rotatebox{90}{$<1$}   & \rotatebox{90}{[1,1.6)} & \rotatebox{90}{[1.6,2.05)}& \rotatebox{90}{[2.05,2.7)} & \rotatebox{90}{[2.7,4.2)} & \rotatebox{90}{$\geq 4.2$}   \\
\midrule
Accuracy & 1 & 1 & 0 & 0 & 0 & 0 \\
Addition &  8 & 17 & 14 & 10 & 11 & 16 \\
Mistranslation & 76 & 82 & 70 & 70 & 58 & 77 \\
Non-existing WF & 2 & 6 & 5 & 4 & 5 & 4 \\
Omission & 15 &  7 &  5 & 14 & 15 & 11 \\
Overly litteral &  6 & 17 & 16 & 16 & 13 & 10 \\
\midrule
Total accuracy & 108 & 130 & 110 & 114 & 102 & 118 \\
\midrule
Fluency & 4 & 1 & 3 & 3 & 4 & 2 \\
Duplication & 0 & 0 & 1 & 5 & 0 & 5 \\
Grammar &  8 &  9 &  7 & 13 &  9 & 11 \\
Typography & 12 &  4 &  5 &  5 & 10 &  5 \\
Unintelligible & 1 & 0 & 0 & 0 & 1 & 0 \\
Word order &  7 &  5 &  8 & 17 & 10 & 18 \\
\midrule
Total fluency & 32 & 19 & 24 & 43 & 34 & 41 \\
\midrule
Total & 140 & 149 & 134 & 157 & 136 & 159 \\
\bottomrule
\end{tabular}


==> tables/archive/diff_pa_offline_ende.tex <==
\begin{tabular}{lrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | PA-offline}\\
\midrule
%Difficulty & $<1$    & [1,1.6)    & [1.6,2.05) & [2.05,2.7) & [2.7,4.2)  & $\geq 4.2$   \\
%\midrule
Accuracy & 0 & 0 & 0 & 0 & 0 & 0 \\
Addition & 10 &  3 &  2 &  5 &  5 &  5 \\
Mistranslation & 41 & 39 & 32 & 43 & 53 & 37 \\
Non-existing WF & 5 & 6 & 8 & 8 & 5 & 7 \\
Omission & 21 & 11 & 13 & 18 & 14 & 22 \\
Overly litteral & 22 & 20 & 18 & 23 & 30 & 37 \\
\midrule
Total accuracy &  99 &  79 &  73 &  97 & 107 & 108 \\
\midrule
Fluency & 5 & 5 & 8 & 3 & 1 & 4 \\
Duplication & 2 & 0 & 1 & 1 & 0 & 1 \\
Grammar & 46 & 25 & 26 & 33 & 25 & 43 \\
Typography &  9 &  4 & 12 & 12 &  5 & 10 \\
Unintelligible & 1 & 0 & 1 & 0 & 1 & 1 \\
Word order &  5 &  3 &  7 &  5 &  9 & 17 \\
\midrule
Total fluency & 68 & 37 & 55 & 54 & 41 & 76 \\
\midrule
Total & 167 & 116 & 128 & 151 & 148 & 184 \\
\bottomrule
\end{tabular}


==> tables/archive/diff_pa_online_deen.tex <==
\begin{tabular}{Hrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | PA-online}\\
\midrule
    Difficulty & \rotatebox{90}{$<1$}   & \rotatebox{90}{[1,1.6)} & \rotatebox{90}{[1.6,2.05)}& \rotatebox{90}{[2.05,2.7)} & \rotatebox{90}{[2.7,4.2)} & \rotatebox{90}{$\geq 4.2$}   \\
\midrule
Accuracy & 0 & 1 & 0 & 0 & 0 & 0 \\
Addition & 20 & 20 & 31 & 10 & 29 & 33 \\
Mistranslation &  82 & 102 & 101 &  90 & 109 & 103 \\
Non-existing WF & 1 & 5 & 3 & 1 & 6 & 1 \\
Omission & 10 & 12 & 18 & 23 & 25 & 25 \\
Overly litteral &  8 & 24 & 15 & 18 & 18 & 12 \\
\midrule
Total accuracy & 121 & 164 & 168 & 142 & 187 & 174 \\
\midrule
Fluency & 4 & 3 & 3 & 3 & 3 & 4 \\
Duplication &  8 &  1 &  2 &  4 &  4 & 13 \\
Grammar & 15 & 11 &  6 & 10 & 20 &  3 \\
Typography &  8 &  7 &  4 &  8 & 12 &  3 \\
Unintelligible & 0 & 1 & 0 & 0 & 1 & 1 \\
Word order & 10 &  9 & 20 & 15 & 28 & 23 \\
\midrule
Total fluency & 45 & 32 & 35 & 40 & 68 & 47 \\
\midrule
Total & 166 & 196 & 203 & 182 & 255 & 221 \\
\bottomrule
\end{tabular}


==> tables/archive/diff_pa_online_ende.tex <==
\begin{tabular}{Hrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | PA-online}\\
\midrule
%Difficulty & $<1$    & [1,1.6)    & [1.6,2.05) & [2.05,2.7) & [2.7,4.2)  & $\geq 4.2$   \\
%\midrule
Accuracy & 0 & 0 & 0 & 0 & 0 & 0 \\
Addition &  4 &  7 & 10 & 12 & 13 & 20 \\
Mistranslation & 38 & 47 & 40 & 44 & 48 & 43 \\
Non-existing WF & 12 &  8 &  9 & 11 &  8 & 10 \\
Omission & 12 &  8 &  4 & 13 & 19 & 18 \\
Overly litteral & 28 & 19 & 24 & 27 & 37 & 44 \\
\midrule
Total accuracy &  94 &  89 &  87 & 107 & 125 & 135 \\
\midrule
Fluency & 3 & 5 & 6 & 2 & 1 & 4 \\
Duplication & 0 & 1 & 0 & 5 & 3 & 6 \\
Grammar & 49 & 36 & 36 & 39 & 45 & 55 \\
Typography & 15 & 12 & 16 & 13 & 15 & 21 \\
Unintelligible & 1 & 0 & 0 & 1 & 4 & 2 \\
Word order &  9 &  9 &  9 & 12 & 21 & 25 \\
\midrule
Total fluency &  77 &  63 &  67 &  72 &  89 & 113 \\
\midrule
Total & 171 & 152 & 154 & 179 & 214 & 248 \\
\bottomrule
\end{tabular}


==> tables/archive/diff_tf_offline_deen.tex <==
\begin{tabular}{Hrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | TF-offline}\\
\midrule
Difficulty & \rotatebox{90}{$<1$}   & \rotatebox{90}{[1,1.6)} & \rotatebox{90}{[1.6,2.05)}& \rotatebox{90}{[2.05,2.7)} & \rotatebox{90}{[2.7,4.2)} & \rotatebox{90}{$\geq 4.2$}   \\
\midrule
Accuracy & 0 & 1 & 0 & 0 & 0 & 1 \\
Addition & 16 &  8 & 15 & 20 & 15 & 21 \\
Mistranslation & 70 & 76 & 79 & 78 & 76 & 78 \\
Non-existing WF & 2 & 2 & 1 & 2 & 3 & 4 \\
Omission & 16 & 10 & 12 & 16 & 31 & 11 \\
Overly litteral & 11 & 12 &  8 &  7 &  7 &  7 \\
\midrule
Total accuracy & 115 & 109 & 115 & 123 & 132 & 122 \\
\midrule
Fluency & 3 & 2 & 2 & 4 & 2 & 1 \\
Duplication & 1 & 5 & 1 & 1 & 6 & 8 \\
Grammar & 11 &  5 &  3 &  6 &  6 &  5 \\
Typography & 8 & 6 & 2 & 5 & 7 & 5 \\
Unintelligible & 0 & 0 & 0 & 1 & 1 & 0 \\
Word order &  5 &  6 &  9 & 12 & 19 & 15 \\
\midrule
Total fluency & 28 & 24 & 17 & 29 & 41 & 34 \\
\midrule
Total & 143 & 133 & 132 & 152 & 173 & 156 \\
\bottomrule
\end{tabular}


==> tables/archive/diff_tf_offline_ende.tex <==
\begin{tabular}{Hrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | TF-offline}\\
\midrule
%Difficulty & $<1$    & [1,1.6)    & [1.6,2.05) & [2.05,2.7) & [2.7,4.2)  & $\geq 4.2$   \\
%\midrule
Accuracy & 0 & 0 & 0 & 0 & 0 & 0 \\ 
Addition &  6 &  3 &  4 & 10 &  6 &  6 \\ 
Mistranslation & 36 & 38 & 35 & 27 & 28 & 38 \\ 
Non-existing WF &  5 &  7 &  5 &  8 &  6 & 12 \\ 
Omission & 22 & 25 & 21 & 26 & 19 & 13 \\ 
Overly litteral & 13 &  9 & 16 & 19 & 31 & 25 \\ 
\midrule
Total accuracy & 82 & 82 & 81 & 90 & 90 & 94 \\ 
\midrule
Fluency & 3 & 2 & 5 & 4 & 3 & 3 \\ 
Duplication & 3 & 1 & 2 & 2 & 2 & 3 \\ 
Grammar & 27 & 17 & 19 & 22 & 19 & 38 \\ 
Typography & 17 &  5 &  3 &  6 & 10 &  8 \\ 
Unintelligible & 1 & 1 & 2 & 1 & 4 & 2 \\ 
Word order &  5 &  3 &  0 &  4 & 12 & 13 \\ 
\midrule
Total fluency & 56 & 29 & 31 & 39 & 50 & 67 \\ 
\midrule
Total & 138 & 111 & 112 & 129 & 140 & 161 \\ 
\bottomrule
\end{tabular}


==> tables/archive/diff_tf_online_deen.tex <==
\begin{tabular}{Hrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | TF-online}\\
\midrule
Difficulty & \rotatebox{90}{$<1$}   & \rotatebox{90}{[1,1.6)} & \rotatebox{90}{[1.6,2.05)}& \rotatebox{90}{[2.05,2.7)} & \rotatebox{90}{[2.7,4.2)} & \rotatebox{90}{$\geq 4.2$}   \\
\midrule
Accuracy & 2 & 0 & 1 & 0 & 0 & 0 \\
Addition & 20 & 17 & 26 & 18 & 34 & 45 \\
Mistranslation &  80 &  82 & 112 &  93 & 108 &  97 \\
Non-existing WF & 1 & 4 & 2 & 0 & 5 & 4 \\
Omission & 23 & 17 & 17 & 19 & 27 & 24 \\
Overly litteral &  5 & 25 & 14 & 15 & 12 & 10 \\
\midrule
Total accuracy & 131 & 145 & 172 & 145 & 186 & 180 \\
\midrule
Fluency & 3 & 2 & 3 & 5 & 5 & 2 \\
Duplication & 16 & 17 & 18 & 30 & 33 & 30 \\
Grammar & 9 & 9 & 3 & 5 & 6 & 2 \\
Typography & 11 & 11 & 11 &  5 & 14 &  7 \\
Unintelligible & 1 & 0 & 0 & 0 & 1 & 0 \\
Word order &  8 &  4 & 14 & 13 & 16 & 23 \\
\midrule
Total fluency & 48 & 43 & 49 & 58 & 75 & 64 \\
\midrule
Total & 179 & 188 & 221 & 203 & 261 & 244 \\
\bottomrule
\end{tabular}


==> tables/archive/diff_tf_online_ende.tex <==
\begin{tabular}{Hrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | TF-online}\\
\midrule
%Difficulty & $<1$    & [1,1.6)    & [1.6,2.05) & [2.05,2.7) & [2.7,4.2)  & $\geq 4.2$   \\
%\midrule
Accuracy & 0 & 0 & 0 & 1 & 0 & 0 \\
Addition &  9 & 12 & 14 & 18 & 22 & 22 \\
Mistranslation & 41 & 34 & 35 & 37 & 54 & 59 \\
Non-existing WF & 14 & 13 &  5 &  4 &  8 & 10 \\
Omission & 15 & 13 & 20 & 25 & 24 & 17 \\
Overly litteral & 19 & 21 & 16 & 21 & 24 & 24 \\
\midrule
Total accuracy &  98 &  93 &  90 & 106 & 132 & 132 \\
\midrule
Fluency & 3 & 3 & 8 & 5 & 2 & 3 \\
Duplication & 15 &  4 & 13 & 11 & 13 & 15 \\
Grammar & 34 & 32 & 40 & 35 & 38 & 43 \\
Typography & 13 & 15 & 17 &  7 & 10 & 16 \\
Unintelligible & 1 & 1 & 0 & 2 & 4 & 3 \\
Word order & 17 &  9 &  8 &  9 & 11 & 20 \\
\midrule
Total fluency &  83 &  64 &  86 &  69 &  78 & 100 \\
\midrule
Total & 181 & 157 & 176 & 175 & 210 & 232 \\
\bottomrule
\end{tabular}


==> tables/archive/difficulty.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
%\cmidrule[.8pt]{3-8}
&        & \multicolumn{6}{c}{\ld} \\
\cmidrule[.6pt]{2-8}
           &  Total & <0 & 0-2 & 2-4 & 4-6 & 6-8 & $\geq$8 \\
\midrule
De$\sto$En &   6750 & 15 & 3936 & 2082 & 485 & 133 & 99\\
De$\sto$En - filtered  ($\lx\in[11,27]$)
           &  3477 &  9 & 2134 & 1172 & 144 & 16 & 2 \\
De$\sto$En - for human annotation
           &  200   &  8 & 93 & 68 & 21 & 9 & 1 \\
\midrule
En$\sto$De &   6750 & 9 & 3878 & 2249 & 417 & 109 & 88 \\
En$\sto$De - filtered  ($\lx\in[11,26]$)
           &   3437 & 4 & 2019 & 1253 & 151 & 8 & 2 \\
En$\sto$De - for human annotation 
           &    200 & 3 & 95 & 64 & 28 & 8 & 2 \\
\bottomrule
\end{tabular}



==> tables/archive/ende_errors_raw_pt.tex <==
\begin{tabular}{Hrrr|rrr|}
\toprule
& \multicolumn{6}{c|}{En$\sto$De}\\
\midrule
& \multicolumn{3}{c|}{PA} & \multicolumn{3}{c|}{TF}\\
\midrule
System & Offline & Online & $\Delta\%$ & Offline & Online & $\Delta\%$\\
\midrule
Accuracy & 0.00 & 0.00 & - & 0.00 & 0.03 & $\infty$\\
Addition &   0.91 &   2.00 & 120 &   1.06 &   2.94 & 177 \\
Mistranslation &  7.44 &  7.89 &  6 &  6.13 &  7.89 & 29 \\
Non-existing WF &  1.18 &  1.76 & 49 &  1.31 &  1.64 & 26 \\
Omission &   3.01 &   2.25 & -25 &   3.82 &   3.46 &  -10 \\
Overly litteral &  4.55 &  5.43 & 19 &  3.43 &  3.79 & 11 \\
\midrule
Total accuracy & 17.09 & 19.33 & 13 & 15.75 & 19.76 & 25 \\
\midrule
Fluency &   0.79 &   0.64 & -19 &   0.61 &   0.73 &  20 \\
Duplication &   0.15 &   0.46 & 200 &   0.39 &   2.15 & 446 \\
Grammar &  6.01 &  7.89 & 31 &  4.31 &  6.74 & 56 \\
Typography &  1.58 &  2.79 & 77 &  1.49 &  2.37 & 59 \\
Unintelligible &   0.12 &   0.24 & 100 &   0.33 &   0.33 &   0 \\
Word order &   1.40 &   2.58 &  85 &   1.12 &   2.27 & 100 \\
\midrule
Total fluency & 10.05 & 14.60 & 45 &  8.26 & 14.57 & 76 \\
\midrule
Total & 27.13 & 33.93 & 25 & 24.01 & 34.32 & 43 \\
%Hyplength & 3440 & 3625 & 5.378 & 3399 & 3708 & 9.091 \\
%Reflength & 3295 & 3295 &    0 & 3295 & 3295 &    0 \\

\bottomrule
\end{tabular}


==> tables/archive/ende_errors_span.tex <==
\begin{tabular}{Hrrr|rrr}
\toprule
& \multicolumn{6}{c}{En$\sto$De}\\
\midrule
& \multicolumn{3}{c|}{PA} & \multicolumn{3}{c}{TF}\\
\midrule
System & Offline & Online & $\Delta\%$ & Offline & Online & $\Delta\%$\\
\midrule
Accuracy &   0 &   0 & 0 &   0 &   1 & - \\
Addition &  60 & 140 & \bad133 &  94 & 233 & \bad148 \\
Mistranslation & 414 & 439 &   6 & 358 & 481 &  34 \\
Non-existing WF & 62 & 83 & 34 & 58 & 76 & 31 \\
Omission &  98 &  78 & \good-20 & 117 & 110 &  \good-6 \\
Overly litteral & 389 & 463 &  19 & 285 & 341 &  20 \\
\midrule
Total accuracy & 634 & 740 &  17 & 627 & 901 &  44 \\
\midrule
Fluency &  53 &  44 & \good-17 &  38 &  54 &  42 \\
Duplication &  10 &  40 & \bad300 &  35 & 154 & \bad340 \\
Grammar & 293 & 378 &  29 & 209 & 321 &  \bad54 \\
Typography &  86 & 135 &  \bad57 &  80 & 123 &  \bad54 \\
Unintelligible &  42 &  68 &  \bad62 & 106 & 113 &   7 \\
Word order &  86 & 152 &  \bad77 &  68 & 147 & \bad116 \\
\midrule
Total fluency &  959 & 1280 &   33 &  821 & 1253 &   \bad53 \\
\midrule
Total & 1593 & 2020 &   27 & 1448 & 2154 &   49 \\
\bottomrule
\end{tabular}


==> tables/archive/length_stats_deen.tex <==
\begin{tabular}{llrrr}
\toprule
System & bin & \#segments & \makecell[r]{\#hypothesis\\tokens} & \makecell[r]{\#reference\\tokens \\ \maha{Denominator}}\\ 
\midrule
PA-offline & [0,14) & 108 & 664 & 597 \\ 
PA-offline & [14,16) &  78 & 565 & 565 \\ 
PA-offline & [16,19) &  78 & 696 & 673 \\ 
PA-offline & [19,22) &  56 & 563 & 559 \\ 
PA-offline & [22,24) &  42 & 451 & 473 \\ 
PA-offline & $\geq 24$ &  38 & 462 & 511 \\ 
\midrule
PA-online & [0,14) & 108 & 665 & 597 \\ 
PA-online & [14,16) &  78 & 586 & 565 \\ 
PA-online & [16,19) &  78 & 725 & 673 \\ 
PA-online & [19,22) &  56 & 542 & 559 \\ 
PA-online & [22,24) &  42 & 474 & 473 \\ 
PA-online & $\geq 24$ &  38 & 468 & 511 \\ 
\midrule
TF-offline & [0,14) & 108 & 633 & 597 \\ 
TF-offline & [14,16) &  78 & 573 & 565 \\ 
TF-offline & [16,19) &  78 & 678 & 673 \\ 
TF-offline & [19,22) &  56 & 554 & 559 \\ 
TF-offline & [22,24) &  42 & 447 & 473 \\ 
TF-offline & $\geq 24$ &  38 & 443 & 511 \\ 
\midrule
TF-online & [0,14) & 108 & 688 & 597 \\ 
TF-online & [14,16) &  78 & 621 & 565 \\ 
TF-online & [16,19) &  78 & 772 & 673 \\ 
TF-online & [19,22) &  56 & 579 & 559 \\ 
TF-online & [22,24) &  42 & 470 & 473 \\ 
TF-online & $\geq 24$ &  38 & 482 & 511 \\ 
\bottomrule
\end{tabular}


==> tables/archive/mt_pa_offline_deen.tex <==
\begin{tabular}{r|rrrrrrr|rrr}
\toprule
& \multicolumn{9}{c}{\#mt-erros}\\
    $\ly$ & 0 & 1 & 2 & 3 & 4 & 5 & 6 & \#segments & \#tokens & in-bin (2 annotations)\\ 
\midrule
8 & 4 & 3 & 2 & 0 & 1 & 0 & 0 & 10 & 80 & \multirow{6}{*}{1194}\\
9 & 5 & 2 & 3 & 2 & 0 & 0 & 0 & 12 & 108 & \\
10 & 7 & 5 & 2 & 0 & 0 & 0 & 0 & 14 & 140& \\
11 & 10 & 5 & 6 & 0 & 1 & 0 & 0 & 22 & 242& \\
12 & 4 & 12 & 8 & 2 & 0 & 0 & 0 & 26 & 312 & \\
13 & 13 & 8 & 2 & 1 & 0 & 0 & 0 & 24 & 312 & \\
\midrule
14 & 14 & 15 & 7 & 1 & 1 & 1 & 1 & 40 & 560& \multirow{2}{*}{1130}\\
15 & 12 & 12 & 11 & 2 & 0 & 1 & 0 & 38 & 570& \\
\midrule
16 & 2 & 8 & 5 & 1 & 0 & 0 & 0 & 16 & 256 & \multirow{3}{*}{1346}\\
17 & 14 & 10 & 2 & 0 & 0 & 0 & 0 & 26 & 442&  \\
18 & 10 & 9 & 7 & 8 & 1 & 1 & 0 & 36 & 648&  \\
\midrule
19 & 13 & 6 & 1 & 1 & 1 & 0 & 0 & 22 & 418 & \multirow{3}{*}{1118}\\
20 & 8 & 2 & 2 & 1 & 1 & 0 & 0 & 14 & 280& \\
21 & 7 & 5 & 3 & 4 & 1 & 0 & 0 & 20 & 420& \\
\midrule
22 & 6 & 9 & 3 & 2 & 0 & 0 & 0 & 20  & 440& \multirow{2}{*}{946}\\
23 & 8 & 7 & 2 & 4 & 1 & 0 & 0 & 22 & 506& \\
\midrule
24 & 0 & 2 & 2 & 2 & 0 & 0 & 0 & 6 & 144&\multirow{9}{*}{1022} \\
25 & 4 & 3 & 1 & 0 & 0 & 0 & 0 & 8 & 200& \\
26 & 4 & 2 & 0 & 1 & 1 & 0 & 0 & 8 & 208& \\
27 & 1 & 2 & 1 & 0 & 0 & 0 & 0 & 4 & 108& \\
28 & 4 & 0 & 0 & 0 & 0 & 0 & 0 & 4 & 112& \\
29 & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 58 & \\
30 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 2 & 60 & \\
31 & 0 & 0 & 0 & 1 & 1 & 0 & 0 & 2 & 62 & \\
35 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 2 & 70 & \\
\midrule
Sum & 153 & 128 & 71 & 34 & 10 & 3 & 1 & & &\\
\bottomrule
\end{tabular}


==> tables/archive/reflen_pa_offline_deen.tex <==
\begin{tabular}{lrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | PA-offline}\\
\midrule
Reference length & \rotatebox{90}{$<14$}   & \rotatebox{90}{[14,16)} & \rotatebox{90}{[16,19)}& \rotatebox{90}{[19,22)} & \rotatebox{90}{[22,24)} & \rotatebox{90}{$\geq 24$}   \\
\midrule
%Accuracy & 0 & 0 & 0 & 0 & 1 & 1 \\
%Addition & 25 & 10 & 12 & 14 &  6 &  9 \\
%Mistranslation & 104 &  92 &  91 &  55 &  48 &  43 \\
%Non-existing WF & 7 & 8 & 6 & 5 & 0 & 0 \\
%Omission & 12 & 11 & 15 &  9 & 13 &  7 \\
%Overly litteral & 14 & 16 & 20 &  8 & 11 &  9 \\
%\midrule
%Total accuracy & 162 & 137 & 144 &  91 &  79 &  69 \\
%\midrule
%Fluency & 3 & 1 & 4 & 3 & 1 & 5 \\
%Duplication & 0 & 1 & 6 & 3 & 0 & 1 \\
%Grammar & 12 & 13 & 10 & 10 &  6 &  6 \\
%Typography &  8 &  7 & 10 &  5 &  6 &  5 \\
%Unintelligible & 1 & 0 & 0 & 1 & 0 & 0 \\
%Word order &  6 & 14 & 15 & 12 &  9 &  9 \\
%\midrule
%Total fluency & 30 & 36 & 45 & 34 & 22 & 26 \\
%\midrule
%Total & 192 & 173 & 189 & 125 & 101 &  95 \\
\midrule
\#tokens& 1194 & 1130 & 1346 & 1118 &  946 & 1022 \\
\#segments & 108 &  78 &  78 &  56 &  42 &  38 \\
\bottomrule
\end{tabular}


==> tables/archive/reflen_pa_offline_ende.tex <==
\begin{tabular}{lrrrrrr}
%\toprule
& \multicolumn{6}{c}{En$\sto$De | PA-offline}\\
\midrule
Reference length & \rotatebox{90}{$<13$}   & \rotatebox{90}{[13,16)} & \rotatebox{90}{[16,18)}& \rotatebox{90}{[18,21)} & \rotatebox{90}{[21,24)} & \rotatebox{90}{$\geq 24$}   \\
\midrule
Accuracy & 0 & 0 & 0 & 0 & 0 & 0 \\
Addition & 7 & 3 & 4 & 5 & 6 & 5 \\
Mistranslation & 55 & 33 & 34 & 59 & 31 & 33 \\
Non-existing WF & 9 & 5 & 8 & 9 & 5 & 3 \\
Omission & 13 & 17 & 10 & 26 & 17 & 16 \\
Overly litteral & 28 & 22 & 20 & 31 & 22 & 27 \\
\midrule
Total accuracy & 112 &  80 &  76 & 130 &  81 &  84 \\
\midrule
Fluency & 3 & 2 & 3 & 7 & 6 & 5 \\
Duplication & 0 & 0 & 1 & 1 & 1 & 2 \\
Grammar & 25 & 24 & 36 & 45 & 36 & 32 \\
Typography &  7 &  5 & 14 & 10 &  8 &  8 \\
Unintelligible & 0 & 0 & 0 & 2 & 1 & 1 \\
Word order & 13 &  5 &  9 &  7 &  6 &  6 \\
\midrule
Total fluency & 48 & 36 & 63 & 72 & 58 & 54 \\
\midrule
Total & 160 & 116 & 139 & 202 & 139 & 138 \\
\midrule
CountTok & 1082 &  996 &  912 & 1324 & 1230 & 1046 \\
Count & 106 &  72 &  56 &  70 &  56 &  40 \\
\bottomrule
\end{tabular}


==> tables/archive/rpos_pa_offline_deen.tex <==
\begin{tabular}{lrrrrr}
\toprule
& \multicolumn{5}{c}{De$\sto$En | PA-offline}\\
\midrule
Relative position & \rotatebox{90}{[0,0.2]} & \rotatebox{90}{(0.2,0.4]}& \rotatebox{90}{(0.4,0.6]}& \rotatebox{90}{(0.6,0.8]} & \rotatebox{90}{(0.8,1]}\\ 
\midrule
Accuracy & 50 & 50 &  0 &  0 &  0 \\
Addition & 12 & 16 & 21 & \bf32 & 19 \\
Mistranslation & 12 & 21 & 26 & 26 & 14 \\
Non-existing WF & 16 & 18 & \bf32 & 16 & 18 \\
Omission & 12 & 19 & 26 & 25 & 18 \\
Overly litteral &  9 & 23 & 18 & \bf33 & 17 \\
\midrule
Total accuracy & 12 & 20 & 26 & 26 & 15 \\
\midrule
Fluency & 18 & 31 & 20 & 22 &  8 \\
Duplication &  6 &  6 & \bf56 & \bf31 &  0 \\
Grammar & 12 & 16 & 23 & \bf36 & 13 \\
Typography & 14 & 26 & 19 & 27 & 14 \\
Unintelligible & 18 & \bf36 & 18 & 18 &  9 \\
Word order & 10 & 15 & 25 & \bf32 & 18 \\
\midrule
Total fluency & 12 & 20 & 22 & \bf31 & 14 \\
\midrule
Total & 12 & 20 & 24 & \bf28 & 15 \\
\bottomrule
\end{tabular}


==> tables/archive/rpos_pa_offline_ende.tex <==
\begin{tabular}{lrrrrr}
%\toprule
& \multicolumn{5}{c}{En$\sto$De | PA-offline}\\
\midrule
%Relative position & \rotatebox{90}{[0,0.2]} & \rotatebox{90}{(0.2,0.4]}& \rotatebox{90}{(0.4,0.6]}& \rotatebox{90}{(0.6,0.8]} & \rotatebox{90}{(0.8,1]}\\ 
%\midrule
Accuracy & - & - & - & - & -\\
Addition &  8 & 23 & \bf28 & \bf30 & 10 \\
Mistranslation &  9 & 23 & 24 & 26 & 17 \\
Non-existing WF &  3 & \bf47 &  8 & 24 & 18 \\
Omission &  8 & 19 & 31 & 24 & 17 \\
Overly litteral & 10 & 20 & 27 & 26 & 17 \\
\midrule
Total accuracy &  9 & 25 & 24 & 26 & 17 \\
\midrule
Fluency & 17 & 23 & 26 & \bf28 &  6 \\
Duplication &  0 & 30 & 10 &  0 & \bf60 \\
Grammar &  6 & 20 & 29 & \bf31 & 14 \\
Typography &  9 & 19 & \bf30 & \bf31 & 10 \\
Unintelligible &  0 & 21 & \bf33 & 26 & 19 \\
Word order & 12 & 23 & 15 & \bf30 & 20 \\
\midrule
Total fluency &  8 & 21 & 27 & \bf28 & 16 \\
\midrule
Total &  8 & 22 & 26 & 27 & 16 \\
\bottomrule
\end{tabular}


==> tables/archive/rpos_pa_online_deen.tex <==
\begin{tabular}{Hrrrrr}
\toprule
& \multicolumn{5}{c}{De$\sto$En | PA-online}\\
\midrule
Relative position & \rotatebox{90}{[0,0.2]} & \rotatebox{90}{(0.2,0.4]}& \rotatebox{90}{(0.4,0.6]}& \rotatebox{90}{(0.6,0.8]} & \rotatebox{90}{(0.8,1]}\\ 

\midrule
Accuracy & 100 &  0 &  0 &  0 &  0 \\
Addition &  8 & 22 & 20 & \bf33 & 16 \\
Mistranslation & 12 & 22 & 25 & \bf29 & 13 \\
Non-existing WF & 14 & 24 & 14 & \bf31 & 17 \\
Omission & 16 & 11 & 25 & 27 & 21 \\
Overly litteral & 12 & 20 & 24 & \bf32 & 13 \\
\midrule
Total accuracy & 12 & 21 & 24 & \bf29 & 14 \\
\midrule
Fluency & 18 & 26 & \bf29 & 19 &  8 \\
Duplication &  8 & 13 & 19 & \bf36 & 25 \\
Grammar & 15 & 25 & 24 & 24 & 11 \\
Typography & 16 & 29 & 24 & 19 & 13 \\
Unintelligible &  7 & 17 & 17 & \bf34 & 24 \\
Word order &  8 & 22 & 21 & 22 & 27 \\
\midrule
Total fluency & 12 & 22 & 23 & 26 & 17 \\
\midrule
Total & 12 & 21 & 23 & \bf28 & 15 \\
\bottomrule
\end{tabular}


==> tables/archive/rpos_pa_online_ende.tex <==
\begin{tabular}{Hrrrrr}
%\toprule
& \multicolumn{5}{c}{En$\sto$De | PA-online}\\
\midrule
%Relative position & \rotatebox{90}{[0,0.2]} & \rotatebox{90}{(0.2,0.4]}& \rotatebox{90}{(0.4,0.6]}& \rotatebox{90}{(0.6,0.8]} & \rotatebox{90}{(0.8,1]}\\ 
%\midrule
Accuracy & - & - & - &  - &  - \\
Addition & 13 & 26 & 19 & 26 & 17 \\
Mistranslation &  9 & 24 & \bf28 & 24 & 15 \\
Non-existing WF & 11 & \bf37 & 19 & 17 & 16 \\
Omission & 12 & 14 & \bf29 & 17 & \bf28 \\
Overly litteral & 10 & 18 & 27 & \bf29 & 16 \\
\midrule
Total accuracy & 10 & 25 & 25 & 23 & 17 \\
\midrule
Fluency & 14 & 14 & 25 & \bf34 & 14 \\
Duplication &  8 & 22 & 20 & \bf28 & 22 \\
Grammar & 11 & 25 & \bf28 & 24 & 12 \\
Typography & 12 & 27 & 24 & \bf32 &  5 \\
Unintelligible & 10 & 28 & \bf31 & 19 & 12 \\
Word order & 13 & 24 & 22 & 27 & 14 \\
\midrule
Total fluency & 11 & 22 & 26 & 27 & 13 \\
\midrule
Total & 11 & 23 & 26 & 26 & 15 \\
\bottomrule
\end{tabular}


==> tables/archive/rpos_tf_offline_deen.tex <==
\begin{tabular}{Hrrrrr}
\toprule
& \multicolumn{5}{c}{De$\sto$En | TF-offline}\\
\midrule
Relative position & \rotatebox{90}{[0,0.2]} & \rotatebox{90}{(0.2,0.4]}& \rotatebox{90}{(0.4,0.6]}& \rotatebox{90}{(0.6,0.8]} & \rotatebox{90}{(0.8,1]}\\ 
\midrule
Accuracy & 29 &  0 &  0 & \bf57 & 14 \\
Addition & 14 & 23 & 24 & 25 & 13 \\
Mistranslation & 11 & 20 & 26 & \bf29 & 14 \\
Non-existing WF &  8 &  4 & \bf36 & \bf28 & 24 \\
Omission & 20 & 16 & 22 & \bf34 &  9 \\
Overly litteral &  7 & 23 & 22 & \bf38 & 10 \\
\midrule
Total accuracy & 12 & 20 & 25 & \bf29 & 13 \\
\midrule
Fluency & 28 & 22 & 10 & \bf35 &  5 \\
Duplication & 14 & 17 & \bf40 & 14 & 14 \\
Grammar & 13 & 14 & \bf29 & \bf28 & 16 \\
Typography &  9 & 19 & 21 & \bf28 & 24 \\
Unintelligible & 17 & 17 & 17 & \bf33 & 17 \\
Word order &  9 & 26 & 21 & 25 & 18 \\
\midrule
Total fluency & 11 & 21 & 23 & \bf29 & 15 \\
\midrule
Total & 12 & 20 & 25 & \bf29 & 14 \\
\bottomrule
\end{tabular}


==> tables/archive/rpos_tf_offline_ende.tex <==
\begin{tabular}{Hrrrrr}
%\toprule
& \multicolumn{5}{c}{En$\sto$De | TF-offline}\\
\midrule
%Relative position & \rotatebox{90}{[0,0.2]} & \rotatebox{90}{(0.2,0.4]}& \rotatebox{90}{(0.4,0.6]}& \rotatebox{90}{(0.6,0.8]} & \rotatebox{90}{(0.8,1]}\\ 
%\midrule
Accuracy & - & - & - & - & - \\
Addition & 16 & 19 & \bf28 & 24 & 13 \\
Mistranslation &  9 & 26 & 26 & 21 & 18 \\
Non-existing WF &  0 & 26 & 16 & \bf40 & 19 \\
Omission & 15 & 17 & \bf28 & 22 & 18 \\
Overly litteral &  8 & 16 & 26 & \bf31 & 20 \\
\midrule
Total accuracy & 10 & 23 & 26 & 24 & 17 \\
\midrule
Fluency & 13 & 26 & 24 & 26 & 11 \\
Duplication & 14 &  6 & 26 & \bf40 & 14 \\
Grammar &  8 & 21 & 24 & \bf35 & 12 \\
Typography & 12 & 21 & 32 & \bf30 &  4 \\
Unintelligible &  6 & 23 & \bf31 & 26 & 14 \\
Word order & 22 & 12 & 18 & \bf29 & 19 \\
\midrule
Total fluency & 10 & 18 & 26 & \bf31 & 15 \\
\midrule
Total & 10 & 20 & 26 & \bf28 & 16 \\
\bottomrule
\end{tabular}


==> tables/archive/rpos_tf_online_deen.tex <==
\begin{tabular}{Hrrrrr}
\toprule
& \multicolumn{5}{c}{De$\sto$En | TF-online}\\
\midrule
Relative position & \rotatebox{90}{[0,0.2]} & \rotatebox{90}{(0.2,0.4]}& \rotatebox{90}{(0.4,0.6]}& \rotatebox{90}{(0.6,0.8]} & \rotatebox{90}{(0.8,1]}\\ 
\midrule
Accuracy &  0 & 29 & 29 & 14 & 29 \\
Addition & 10 & 28 & 19 & \bf30 & 13 \\
Mistranslation & 12 & 23 & 23 & 27 & 14 \\
Non-existing WF &  6 &  6 & \bf38 & \bf31 & 19 \\
Omission & 16 & 18 & 15 & \bf30 & 21 \\
Overly litteral & 19 & 21 & 21 & \bf28 & 12 \\
\midrule
Total accuracy & 12 & 23 & 22 & \bf28 & 15 \\
\midrule
Fluency & 11 & 26 & 15 & 27 & 21 \\
Duplication &  7 & 20 & 25 & 24 & 24 \\
Grammar & 14 & 26 & \bf29 & 23 &  8 \\
Typography & 12 & 18 & 25 & \bf35 & 10 \\
Unintelligible & 18 & 18 & \bf29 & 24 & 12 \\
Word order &  6 & 27 & \bf29 & 14 & 24 \\
\midrule
Total fluency & 11 & 22 & 24 & 25 & 18 \\
\midrule
Total & 12 & 23 & 23 & 27 & 16 \\
\bottomrule
\end{tabular}


==> tables/archive/rpos_tf_online_ende.tex <==
\begin{tabular}{Hrrrrr}
%\toprule
& \multicolumn{5}{c}{En$\sto$De | TF-online}\\
\midrule
%Relative position & \rotatebox{90}{[0,0.2]} & \rotatebox{90}{(0.2,0.4]}& \rotatebox{90}{(0.4,0.6]}& \rotatebox{90}{(0.6,0.8]} & \rotatebox{90}{(0.8,1]}\\ 
%\midrule
Accuracy &  0 &  0 & 100 &  0 &  0 \\
Addition & 15 & 24 & 27 & 21 & 13 \\
Mistranslation &  9 & 23 & 26 & 25 & 17 \\
Non-existing WF & 13 & 25 & 20 & 22 & 20 \\
Omission & 13 & 13 & \bf33 & \bf28 & 14 \\
Overly litteral & 15 & 17 & 24 & 27 & 16 \\
\midrule
Total accuracy & 12 & 22 & 27 & 24 & 16 \\
\midrule
Fluency &  6 & 17 & \bf44 & 20 & 13 \\
Duplication &  9 & 26 & \bf29 & 25 & 11 \\
Grammar & 12 & 22 & 27 & 24 & 14 \\
Typography & 18 & 19 & 24 & \bf33 &  6 \\
Unintelligible &  9 & 20 & 27 & \bf28 & 16 \\
Word order & 13 & 24 & 18 & 24 & 20 \\
\midrule
Total fluency & 13 & 21 & 26 & 26 & 14 \\
\midrule
Total & 12 & 21 & 26 & 25 & 15 \\ 
\bottomrule
\end{tabular}


==> tables/automatic.tex <==
\begin{tabular}{lllcccc}
\toprule
& & & \multicolumn{4}{c}{Full}\\
\midrule
& & & BLEU & METEOR & ROUGE-L & RIBES \\
%& & & B & M & R-L & R \\
\midrule
\multirow{4}{*}{De$\sto$En}
& \multirow{2}{*}{Offline} & TF &    31.13 &     32.78  &\bf 63.15 & \ul{84.75} \\
                         & & PA & \bf31.24 & \ul{33.20} &    62.89 &     84.40 \\
\cmidrule{2-7}
& \multirow{2}{*}{Online} & TF &    26.57 & \ul{31.41}& \bf59.51 &     82.17 \\
                        & & PA & \bf26.44 &     30.48&     59.30 &  \bf82.32 \\


\midrule
\multirow{4}{*}{En$\sto$De}
& \multirow{2}{*}{Offline} & TF & \ul{26.60}& \bf27.62 & \ul{58.27}& \ul{81.77} \\
                         & & PA &     26.03 &    27.55 &     57.99 &     81.45\\
\cmidrule{2-7}
& \multirow{2}{*}{Online} & TF &    22.98 & \ul{26.87}&  \bf55.46 &     79.38 \\
                        & & PA & \bf23.04 &     26.63 &     55.41 & \ul{79.90}\\
\bottomrule
\end{tabular}


==> tables/automatic_annot.tex <==
\begin{tabular}{HHHcccc}
\toprule
& & & \multicolumn{4}{c}{Annotated}\\
\midrule
& & & BLEU & METEOR & ROUGE-L & RIBES \\
%& & & B & M & R-L & R \\
\midrule
\multirow{4}{*}{De$\sto$En}
& \multirow{2}{*}{Offline} & TF &    30.98 &    33.35 &    62.15 &  \bf84.89 \\
                         & & PA & \bf31.07 & \bf33.57 &\bf 62.18 &     84.57 \\
\cmidrule{2-7}
& \multirow{2}{*}{Online} & TF & \bf27.12 & \bf31.41& \bf 58.53 &  \bf82.42 \\
                        & & PA &    26.74 &    31.27&     57.90 &     82.20 \\



\midrule
\multirow{4}{*}{En$\sto$De}
& \multirow{2}{*}{Offline} & TF & 24.44 & \bf26.91 & \bf 54.91 & \bf80.85\\
                         & & PA & \bf24.46 &    26.72 &     54.64 &    80.69\\
\cmidrule{2-7}
& \multirow{2}{*}{Online} & TF &    20.83 & \bf25.77 &     51.32 &     77.70 \\
                        & & PA & \bf21.09 &    25.74 &  \bf52.55 & \bf 78.60\\
\bottomrule
\end{tabular}


==> tables/corr/deen.tex <==
\settowidth{\rotheadsize}{SentBLEU}
\begin{tabular}{r|HrrrrrHHHH|HrrrrrHHHH|HrrrrrHHHH|HrrrrrHHHH}
\toprule
& LD & \rothead{\scriptsize TER} & \rothead{\scriptsize SentBLEU} & \rothead{\scriptsize METEOR} & \rothead{\scriptsize BERTScore} & \rothead{\scriptsize$\conf$} & lx & ly & lhyp & \rothead{\scriptsize$\ratio$}
& LD & \rothead{\scriptsize TER} & \rothead{\scriptsize SentBLEU} & \rothead{\scriptsize METEOR} & \rothead{\scriptsize BERTScore} & \rothead{\scriptsize$\conf$} & lx & ly & lhyp & \rothead{\scriptsize$\ratio$}
& LD & \rothead{\scriptsize TER} & \rothead{\scriptsize SentBLEU} & \rothead{\scriptsize METEOR} & \rothead{\scriptsize BERTScore} & \rothead{\scriptsize$\conf$} & lx & ly & lhyp & \rothead{\scriptsize$\ratio$}
& LD & \rothead{\scriptsize TER} & \rothead{\scriptsize SentBLEU} & \rothead{\scriptsize METEOR} & \rothead{\scriptsize BERTScore} & \rothead{\scriptsize$\conf$} & lx & ly & lhyp & \rothead{\scriptsize$\ratio$}\\
\hline
%ac & -0.09 & -0.02 & -0.05 & -0.05 & -0.03 & -0.07 & 0.12 & 0.15 & 0.10 & -0.04 & -0.05 & 0.00 & -0.06 & -0.10 & -0.01 & -0.04 & 0.09 & 0.13 & 0.07 & -0.04 & 0.04 & -0.04 & 0.02 & 0.01 & -0.02 & -0.13 & 0.04 & 0.07 & 0.07 & 0.06 & -0.07 & 0.04 & -0.07 & -0.08 & -0.09 & -0.11 & 0.14 & 0.14 & 0.11 & -0.05 \\ 
ad & 0.08 & 0.26 & -0.16 & -0.12 & -0.28 & \bf-0.42 & 0.01 & 0.01 & 0.21 & 0.39 
   & 0.14 & \bf0.38 & -0.28 & -0.17 & -0.35 & \bf-0.40 & 0.26 & 0.15 & \bf0.38 & 0.24 
   & 0.08 & \bf0.43 & -0.28 & -0.23 & -0.33 & \bf-0.46 & 0.02 & 0.00 & 0.20 & 0.35 
   & 0.26 & \bf0.39 & -0.33 & -0.20 & \bf-0.38 & \bf-0.41 & 0.19 & 0.10 & 0.32 & 0.23 \\ 
mt & 0.07 & 0.36 & -0.41 & -0.38 & \bf-0.54 & \bf-0.45 & 0.05 & 0.05 & 0.13 & 0.17 
   & 0.21 & 0.41 & -0.42 & -0.32 & \bf-0.51 & \bf-0.46 & 0.20 & 0.10 & 0.30 & 0.22 
   & 0.12 & 0.42 & -0.41 & -0.42 & \bf-0.60 & \bf-0.54 & 0.09 & 0.05 & 0.20 & 0.17 
   & 0.21 & 0.40 & -0.41 & -0.42 & \bf-0.54 & \bf-0.50 & 0.12 & 0.10 & 0.24 & 0.23 \\ 
ne & 0.14 & 0.09 & -0.06 & -0.07 & -0.04 & \bf-0.17 & 0.08 & 0.07 & 0.14 & 0.11 
   & 0.10 & 0.13 & -0.04 & -0.00 & -0.09 & \bf-0.16 & \bf0.16 & 0.07 & \bf0.21 & 0.05 
   & 0.11 & 0.10 & -0.08 & -0.06 & -0.10 & -0.04 & 0.17 & \bf0.22 & \bf0.23 & 0.08 
   & 0.16 & \bf0.30 & -0.23 & -0.13 & -0.21 & -0.21 & 0.17 & 0.01 & \bf0.30 & 0.22 \\ 
om & 0.04 & 0.10 & -0.11 & -0.14 & \bf-0.21 & \bf-0.20 & \bf0.20 & 0.12 & 0.09 & \bf-0.19 
   & 0.18 & 0.06 & -0.11 & -0.17 & -0.24 & -0.10 & 0.15 & 0.14 & 0.01 & \bf-0.31 
   & 0.03 & 0.07 & -0.13 & -0.12 & -0.10 & -0.14 & \bf0.20 & 0.14 & 0.10 & \bf-0.19 
   & 0.10 & 0.06 & -0.11 & -0.08 & \bf-0.21 & -0.10 & \bf0.19 & 0.14 & 0.11 & -0.15 \\ 
ol & 0.02 & 0.12 & -0.12 & \bf-0.20 & -0.07 & -0.07 & 0.11 & 0.10 & 0.09 & -0.06 
   & 0.05 & 0.12 & -0.11 & -0.10 & \bf-0.15 & -0.10 & 0.09 & 0.07 & 0.10 & 0.03 
   & -0.01 & 0.14 & -0.12 & -0.13 & \bf-0.15 & \bf-0.15 & 0.05 & 0.07 & 0.10 & 0.09 
   & 0.05 & \bf0.26 & -0.20 & -0.16 & \bf-0.23 & -0.20 & 0.08 & 0.01 & 0.17 & 0.15 \\ 
\hline
ac+ & 0.10 & 0.43 & -0.43 & -0.44 & \bf-0.62 & \bf-0.58 & 0.10 & 0.09 & 0.20 & 0.21 
    & 0.28 & 0.49 & -0.48 & -0.38 & \bf-0.63 & \bf-0.56 & 0.31 & 0.19 & 0.39 & 0.16 
    & 0.14 & 0.53 & -0.48 & -0.46 & \bf-0.63 & \bf-0.66 & 0.14 & 0.09 & 0.27 & 0.21 
    & 0.29 & 0.50 & -0.48 & -0.41 & \bf-0.62 & \bf-0.58 & 0.24 & 0.15 & 0.36 & 0.24 \\ 
\hline
fl & -0.01 & -0.01 & -0.01 & 0.07 & 0.02 & 0.06 & \bf0.17 & \bf0.17 & \bf0.19 & -0.02 
   & 0.03 & 0.03 & -0.04 & 0.03 & -0.05 & -0.00 & \bf0.15 & 0.07 & 0.12 & -0.07 
   & -0.07 & 0.05 & \bf-0.10 & \bf-0.09 & -0.08 & -0.01 & 0.06 & 0.06 & 0.03 & \bf-0.09 
   & -0.01 & -0.00 & -0.04 & -0.01 & 0.02 & 0.00 & 0.08 & 0.09 & 0.07 & -0.04 \\ 
du & 0.14 & 0.09 & -0.06 & -0.07 & -0.04 & \bf-0.17 & 0.08 & 0.07 & 0.14 & 0.11 
   & 0.10 & 0.13 & -0.04 & -0.00 & -0.09 & \bf-0.16 & \bf0.16 & 0.07 & \bf0.21 & 0.05 
   & 0.11 & 0.10 & -0.08 & -0.06 & -0.10 & -0.04 & \bf0.17 & \bf0.22 & \bf0.23 & 0.08 
   & 0.16 & \bf0.30 & -0.23 & -0.13 & -0.21 & -0.21 & 0.17 & 0.01 & \bf0.30 & 0.22 \\ 
gr & 0.10 & 0.08 & -0.12 & -0.01 & -0.08 & -0.01 & 0.07 & 0.07 & 0.10 & 0.05 
   & -0.06 & 0.02 & -0.11 & 0.01 & -0.09 & -0.10 & 0.08 & 0.09 & 0.08 & 0.02 
   & -0.04 & 0.04 & -0.11 & -0.00 & -0.09 & -0.05 & 0.07 & 0.10 & 0.10 & 0.05 
   & -0.13 & -0.02 & -0.04 & 0.04 & -0.03 & -0.10 & 0.04 & 0.03 & 0.04 & 0.02 \\ 
ty & -0.04 & -0.01 & -0.06 & 0.01 & 0.02 & 0.02 & 0.11 & 0.08 & 0.09 & -0.01 
   & -0.03 & 0.05 & -0.06 & -0.02 & -0.05 & 0.09 & 0.05 & 0.05 & 0.07 & 0.08 
   & -0.02 & -0.04 & 0.02 & 0.02 & -0.01 & 0.11 & -0.01 & 0.03 & -0.00 & 0.03 
   & -0.02 & 0.07 & -0.08 & -0.13 & -0.04 & 0.04 & -0.05 & -0.02 & -0.02 & 0.08 \\ 
%un & -0.01 & 0.11 & -0.05 & -0.11 & -0.18 & -0.13 & -0.09 & -0.07 & -0.06 & 0.05 & 0.08 & 0.21 & -0.12 & -0.20 & -0.15 & -0.22 & -0.02 & -0.04 & -0.04 & -0.03 & 0.05 & 0.20 & -0.10 & -0.14 & -0.09 & -0.14 & -0.08 & -0.12 & -0.06 & 0.03 & -0.03 & 0.29 & -0.12 & -0.16 & -0.28 & -0.26 & -0.14 & -0.11 & -0.05 & 0.30 \\ 
wo & 0.15 & 0.07 & -0.05 & -0.06 & -0.09 & -0.10 & \bf0.15 & \bf0.20 & \bf0.19 & 0.06 
   & 0.19 & 0.13 & -0.10 & 0.02 & \bf-0.17 & 0.01 & \bf0.30 & 0.20 & \bf0.28 & -0.05 
   & 0.16 & 0.17 & \bf-0.19 & -0.12 & -0.17 & -0.03 & \bf0.20 & 0.11 & 0.15 & -0.08 
   & 0.22 & 0.11 & -0.09 & -0.11 & -0.13 & -0.02 & \bf0.33 & 0.22 & \bf0.30 & -0.08 \\ 
\hline
fl+ & 0.17 & 0.11 & -0.14 & -0.06 & -0.11 & -0.11 & 0.23 & 0.25 & 0.29 & 0.09 
    & 0.15 & \bf0.20 & -0.17 & -0.00 & \bf-0.23 & -0.09 & 0.36 & 0.24 & 0.36 & 0.01 
    & 0.11 & 0.17 & \bf-0.21 & -0.12 & \bf-0.20 & -0.02 & 0.22 & 0.19 & 0.22 & -0.01 
    & 0.18 & \bf0.30 & \bf-0.24 & -0.17 & \bf-0.24 & -0.18 & 0.27 & 0.11 & 0.36 & 0.16 \\ 
\hline
ac+fl & 0.15 & 0.41 & -0.43 & -0.40 & \bf-0.58 & -0.54 & 0.18 & 0.18 & 0.29 & 0.21 
      & 0.30 & 0.50 & -0.48 & -0.32 & \bf-0.64 & -0.51 & 0.41 & 0.26 & 0.48 & 0.14 
      & 0.17 & 0.54 & -0.51 & -0.46 & \bf-0.64 & -0.59 & 0.21 & 0.16 & 0.32 & 0.18 
      & 0.31 & 0.54 & -0.50 & -0.41 & \bf-0.61 & -0.55 & 0.32 & 0.17 & 0.46 & 0.26 \\ 
\bottomrule
\end{tabular}


==> tables/corr/ende.tex <==
\settowidth{\rotheadsize}{SentBLEU}
\begin{tabular}{r|HrrrrrHHHH|HrrrrrHHHH|HrrrrrHHHH|HrrrrrHHHH}
\toprule
%& LD & \rothead{\scriptsize TER} & \rothead{\scriptsize SentBLEU} & \rothead{\scriptsize METEOR} & \rothead{\scriptsize BERTScore} & \rothead{\scriptsize$\conf$} & lx & ly & lhyp & \rothead{\scriptsize$\ratio$}
%& LD & \rothead{\scriptsize TER} & \rothead{\scriptsize SentBLEU} & \rothead{\scriptsize METEOR} & \rothead{\scriptsize BERTScore} & \rothead{\scriptsize$\conf$} & lx & ly & lhyp & \rothead{\scriptsize$\ratio$}
%& LD & \rothead{\scriptsize TER} & \rothead{\scriptsize SentBLEU} & \rothead{\scriptsize METEOR} & \rothead{\scriptsize BERTScore} & \rothead{\scriptsize$\conf$} & lx & ly & lhyp & \rothead{\scriptsize$\ratio$}
%& LD & \rothead{\scriptsize TER} & \rothead{\scriptsize SentBLEU} & \rothead{\scriptsize METEOR} & \rothead{\scriptsize BERTScore} & \rothead{\scriptsize$\conf$} & lx & ly & lhyp & \rothead{\scriptsize$\ratio$}\\
%\hline
%ac &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.00 & -0.00 & -0.06 & -0.00 & -0.05 & 0.02 & -0.01 & 0.03 & 0.05 & 0.13 \\ 
ad & -0.00 & 0.06 & -0.11 & -0.10 & -0.14 & \bf-0.23 & 0.03 & 0.10 & 0.18 & 0.26 
   & 0.21 & 0.22 & -0.24 & -0.21 & -0.23 & \bf-0.30 & 0.14 & 0.04 & 0.17 & 0.11 
   & 0.05 & 0.18 & -0.09 & -0.13 & -0.19 & \bf-0.34 & 0.03 & 0.03 & 0.20 & 0.33 
   & 0.15 & 0.22 & -0.24 & -0.14 & -0.25 & \bf-0.48 & 0.29 & 0.11 & 0.36 & 0.22 \\ 
mt & 0.04 & 0.14 & -0.27 & -0.25 & -0.28 & \bf-0.43 & 0.13 & 0.16 & 0.14 & 0.05 
   & 0.04 & 0.05 & -0.24 & -0.21 & -0.20 & \bf-0.56 & 0.26 & 0.25 & 0.22 & -0.08 
   & 0.02 & 0.08 & -0.22 & -0.19 & -0.18 & \bf-0.39 & 0.12 & 0.07 & 0.06 & -0.11 
   & 0.26 & 0.22 & -0.26 & -0.27 & -0.31 & \bf-0.44 & 0.24 & 0.16 & 0.21 & -0.00 \\ 
ne & 0.01 & -0.02 & 0.03 & 0.02 & -0.01 & 0.02 & 0.12 & 0.15 & 0.16 & 0.07 
   & 0.14 & \bf0.17 & -0.13 & 0.02 & -0.06 & -0.14 & 0.12 & -0.03 & 0.10 & -0.00 
   & 0.02 & \bf0.26 & -0.21 & -0.23 & -0.19 & \bf-0.27 & 0.05 & -0.01 & 0.12 & 0.11 
   & 0.02 & \bf0.25 & -0.18 & -0.01 & -0.11 & \bf-0.28 & 0.17 & 0.02 & 0.27 & 0.25 \\ 
om & 0.06 & 0.07 & -0.18 & -0.20 & -0.20 & \bf-0.34 & 0.19 & 0.18 & 0.03 & -0.27 
   & 0.13 & 0.17 & -0.25 & -0.24 & -0.25 & \bf-0.35 & 0.13 & 0.07 & 0.05 & -0.17 
   & -0.09 & 0.11 & \bf-0.21 & -0.20 & -0.16 & \bf-0.22 & 0.15 & 0.14 & 0.03 & -0.19 
   & 0.07 & 0.10 & -0.25 & -0.24 & -0.24 & \bf-0.40 & 0.19 & 0.21 & 0.15 & -0.05 \\ 
ol & 0.20 & 0.17 & \bf-0.31 & -0.24 & \bf-0.27 & -0.25 & 0.31 & 0.27 & 0.28 & -0.00 
   & 0.26 & 0.18 & -0.28 & -0.22 & \bf-0.34 & -0.27 & \bf0.33 & 0.22 & 0.33 & 0.04 
   & 0.20 & 0.12 & \bf-0.18 & -0.10 & -0.15 & -0.10 & 0.20 & 0.14 & 0.25 & 0.13 
   & 0.09 & 0.11 & -0.16 & -0.13 & \bf-0.26 & \bf-0.24 & 0.26 & 0.18 & 0.25 & 0.02 \\ 
\hline
ac+ & 0.13 & 0.20 & -0.39 & -0.35 & -0.41 & \bf-0.58 & 0.28 & 0.30 & 0.24 & -0.02 
    & 0.23 & 0.21 & -0.40 & -0.33 & -0.41 & \bf-0.66 & 0.38 & 0.27 & 0.33 & -0.06 
    & 0.10 & 0.20 & -0.35 & -0.27 & -0.32 & \bf-0.51 & 0.23 & 0.18 & 0.23 & 0.02 
    & 0.22 & 0.25 & -0.36 & -0.32 & -0.43 & \bf-0.66 & 0.34 & 0.23 & 0.34 & 0.07 \\ 
\hline
fl & -0.06 & 0.00 & -0.01 & -0.04 & -0.03 & -0.13 & 0.16 & 0.18 & 0.24 & 0.17 
   & -0.02 & 0.02 & -0.08 & -0.07 & -0.12 & -0.12 & 0.17 & 0.16 & 0.19 & 0.08 
   & -0.01 & 0.01 & -0.04 & -0.01 & -0.03 & -0.10 & 0.08 & 0.09 & 0.15 & 0.16 
   & -0.03 & -0.07 & 0.06 & 0.06 & 0.08 & 0.00 & 0.12 & 0.10 & 0.12 & 0.03 \\ 
du & 0.01 & -0.02 & 0.03 & 0.02 & -0.01 & 0.02 & 0.12 & 0.15 & 0.16 & 0.07 
   & 0.14 & \bf0.17 & -0.13 & 0.02 & -0.06 & -0.14 & 0.12 & -0.03 & 0.10 & -0.00 
   & 0.02 & \bf0.26 & -0.21 & -0.23 & -0.19 & \bf-0.27 & 0.05 & -0.01 & 0.12 & 0.11 
   & 0.02 & \bf0.25 & -0.18 & -0.01 & -0.11 & \bf-0.28 & 0.17 & 0.02 & 0.27 & 0.25 \\ 

gr & 0.08 & -0.00 & -0.13 & -0.05 & -0.04 & -0.12 & 0.30 & 0.30 & 0.30 & 0.04 
   & 0.14 & 0.03 & -0.19 & -0.10 & -0.10 & \bf-0.28 & 0.30 & 0.25 & 0.26 & -0.07 
   & 0.18 & 0.01 & -0.08 & -0.06 & -0.05 & -0.01 & 0.24 & 0.24 & 0.22 & -0.00 
   & 0.07 & 0.11 & \bf-0.19 & -0.10 & -0.08 & \bf-0.17 & 0.23 & 0.17 & 0.20 & -0.01 \\ 

ty & 0.03 & 0.10 & -0.06 & -0.07 & -0.09 & -0.07 & 0.08 & 0.13 & 0.12 & 0.07 
   & 0.10 & -0.01 & 0.04 & 0.06 & 0.03 & 0.00 & 0.12 & 0.02 & 0.04 & -0.17 
   & -0.01 & 0.09 & -0.08 & -0.06 & -0.05 & -0.07 & 0.07 & 0.09 & 0.13 & 0.10 
   & 0.05 & -0.00 & -0.02 & 0.03 & 0.02 & -0.06 & 0.11 & 0.06 & 0.11 & 0.01 \\ 

%un & 0.05 & 0.08 & -0.08 & -0.05 & -0.14 & -0.11 & 0.12 & 0.12 & 0.22 & 0.18 & 0.14 & 0.18 & -0.19 & -0.23 & -0.25 & -0.19 & 0.15 & 0.09 & 0.16 & 0.05 & 0.08 & 0.15 & -0.15 & -0.15 & -0.23 & -0.33 & 0.20 & 0.16 & 0.28 & 0.16 & 0.14 & 0.21 & -0.21 & -0.24 & -0.32 & -0.26 & 0.14 & 0.10 & 0.18 & 0.09 \\ 
wo & \bf0.24 & \bf0.23 & \bf-0.24 & -0.15 & \bf-0.26 & -0.13 & 0.14 & 0.02 & 0.09 & -0.07 
   & \bf0.23 & 0.04 & -0.14 & -0.07 & -0.17 & -0.18 & 0.25 & 0.20 & 0.19 & -0.11 
   & \bf0.25 & \bf0.25 & -0.18 & -0.13 & \bf-0.26 & -0.09 & 0.11 & 0.03 & 0.18 & 0.12 
   & 0.08 & 0.19 & \bf-0.21 & -0.15 & \bf-0.20 & \bf-0.20 & 0.16 & 0.10 & 0.20 & 0.13 \\ 

\hline
fl+ & 0.14 & 0.11 & \bf-0.20 & -0.12 & -0.16 & \bf-0.19 & 0.35 & 0.33 & 0.37 & 0.09 
    & 0.25 & 0.08 & -0.22 & -0.11 & -0.18 & \bf-0.32 & 0.40 & 0.29 & 0.33 & -0.13 
    & 0.20 & 0.17 & \bf-0.19 & -0.16 & \bf-0.19 & -0.16 & 0.27 & 0.23 & 0.32 & 0.14 
    & 0.10 & 0.23 & \bf-0.27 & -0.12 & -0.17 & \bf-0.31 & 0.32 & 0.19 & 0.35 & 0.14 \\ 
\hline
ac+fl & 0.17 & 0.21 & -0.39 & -0.32 & -0.39 & \bf-0.53 & 0.40 & 0.41 & 0.39 & 0.04 
      & 0.30 & 0.18 & -0.39 & -0.28 & -0.38 & \bf-0.63 & 0.49 & 0.35 & 0.41 & -0.12 
      & 0.19 & 0.24 & -0.35 & -0.28 & -0.33 & \bf-0.44 & 0.31 & 0.26 & 0.35 & 0.09 
      & 0.21 & 0.30 & -0.39 & -0.28 & -0.38 & \bf-0.62 & 0.42 & 0.27 & 0.44 & 0.13 \\ 
\bottomrule
\end{tabular}


==> tables/corr/pa_offline_deen.tex <==
\begin{tabular}{rrrrrrr|r|rrrrrr|r|r}
\hline
& ac & ad & mt & ne & om & ol & ac+ & fl & du & gr & ty & un & wo & fl+ & ac+fl \\ 
\hline
%LD & -0.09 & 0.08 & 0.07 & \bf0.14 & 0.04 & 0.02 & 0.10 & -0.01 & \bf0.14 & \bf0.10 & -0.04 & -0.01 & 0.15 & 0.17 & 0.15 \\ 
$\downarrow$TER & -0.02 & 0.26 & 0.36 & 0.09 & 0.10 & 0.12 & 0.43 & -0.01 & 0.09 & 0.08 & -0.01 & 0.11 & 0.07 & 0.11 & 0.41 \\ 
$\uparrow$BLEU & -0.05 & -0.16 & \bf-0.41 & -0.06 & -0.11 & -0.12 & -0.43 & -0.01 & -0.06 & \bf-0.12 & -0.06 & -0.05 & -0.05 & -0.14 & -0.43 \\ 
$\uparrow$METEOR & -0.05 & -0.12 & -0.38 & -0.07 & -0.14 & \bf-0.20 & -0.44 & 0.07 & -0.07 & -0.01 & 0.01 & -0.11 & -0.06 & -0.06 & -0.40 \\ 
$\uparrow$BERTScore & -0.03 & -0.28 & \bf-0.54 & -0.04 & \bf-0.21 & -0.07 & \bf-0.62 & 0.02 & -0.04 & -0.08 & 0.02 & \bf-0.18 & -0.09 & -0.11 & \bf-0.58 \\ 
$\uparrow$$\conf$ & -0.07 & \bf-0.42 & \bf-0.45 & \bf-0.17 & \bf-0.20 & -0.07 & \bf-0.58 & 0.06 & \bf-0.17 & -0.01 & 0.02 & -0.13 & -0.10 & -0.11 & \bf-0.54 \\ 
%$\lx$ & 0.12 & 0.01 & 0.05 & 0.08 & \bf0.20 & 0.11 & 0.10 & \bf0.17 & 0.08 & 0.07 & \bf0.11 & -0.09 & 0.15 & \bf0.23 & 0.18 \\ 
%$\ly$ & 0.15 & 0.01 & 0.05 & 0.07 & 0.12 & 0.10 & 0.09 & 0.17 & 0.07 & 0.07 & 0.08 & -0.07 & 0.20 & 0.25 & 0.18 \\ 
%$\lhyp$ & 0.10 & 0.21 & 0.13 & \bf0.14 & 0.09 & 0.09 & 0.20 & \bf0.19 & \bf0.14 & \bf0.10 & 0.09 & -0.06 & \bf0.19 & \bf0.29 & 0.29 \\ 
%$\ratio$ & -0.04 & \bf0.39 & 0.17 & 0.11 & \bf-0.19 & -0.06 & 0.21 & -0.02 & 0.11 & 0.05 & -0.01 & 0.05 & 0.06 & 0.09 & 0.21 \\ 
\hline
\end{tabular}


==> tables/corr/pa_offline_ende.tex <==
\begin{tabular}{r|rrrrrr|r|rrrrrr|r|r}
\hline
& ac & ad & mt & ne & om & ol & ac+ & fl & du & gr & ty & un & wo & fl+& ac+fl\\ 
\hline
LD &  & -0.00 & 0.04 & 0.01 & 0.06 & 0.20 & 0.13 & -0.06 & 0.01 & 0.08 & 0.03 & 0.05 & \bf0.24 & 0.14 & 0.17 \\ 
$\downarrow$TER &  & 0.06 & 0.14 & -0.02 & 0.07 & 0.17 & 0.20 & 0.00 & -0.02 & -0.00 & \bf0.10 & 0.08 & \bf0.23 & 0.11 & 0.21 \\ 
$\uparrow$BLEU &  & -0.11 & -0.27 & 0.03 & -0.18 & \bf-0.31 & -0.39 & -0.01 & 0.03 & -0.13 & -0.06 & -0.08 & \bf-0.24 & -0.20 & \bf-0.39 \\ 
$\uparrow$METEOR &  & -0.10 & -0.25 & 0.02 & -0.20 & -0.24 & -0.35 & -0.04 & 0.02 & -0.05 & -0.07 & -0.05 & -0.15 & -0.12 & \bf-0.32 \\ 
$\uparrow$BERTScore &  & -0.14 & -0.28 & -0.01 & -0.20 & -0.27 & \bf-0.41 & -0.03 & -0.01 & -0.04 & -0.09 & -0.14 & \bf-0.26 & -0.16 & \bf-0.39 \\ 
$\uparrow$$\conf$ &  & \bf-0.23 & \bf-0.43 & 0.02 & \bf-0.34 & -0.25 & \bf-0.58 & -0.13 & 0.02 & -0.12 & -0.07 & -0.11 & -0.13 & -0.19 & \bf-0.53 \\ 
$\lx$ &  & 0.03 & 0.13 & 0.12 & 0.19 & \bf0.31 & 0.28 & 0.16 & 0.12 & \bf0.30 & 0.08 & 0.12 & 0.14 & \bf0.35 & \bf0.40 \\ 
%$\ly$ &  & 0.10 & 0.16 & 0.15 & 0.18 & 0.27 & 0.30 & 0.18 & 0.15 & 0.30 & 0.13 & 0.12 & 0.02 & 0.33 & 0.41 \\ 
$\lhyp$ &  & 0.18 & 0.14 & 0.16 & 0.03 & 0.28 & 0.24 & \bf0.24 & \bf0.16 & \bf0.30 & \bf0.12 & \bf0.22 & 0.09 & \bf0.37 & \bf0.39 \\ 
$\ratio$ &  & \bf0.26 & 0.05 & 0.07 & \bf-0.27 & -0.00 & -0.02 & 0.17 & 0.07 & 0.04 & 0.07 & \bf0.18 & -0.07 & 0.09 & 0.04 \\ 
\hline
\end{tabular}


==> tables/corr/pa_online_deen.tex <==
\begin{tabular}{rrrrrrr|r|rrrrrr|r|r}
\hline
& ac & ad & mt & ne & om & ol & ac+ & fl & du & gr & ty & un & wo & fl+ & ac+fl \\ 
\hline
LD & -0.05 & 0.14 & 0.21 & 0.10 & 0.18 & 0.05 & 0.28 & 0.03 & 0.10 & -0.06 & -0.03 & 0.08 & 0.19 & 0.15 & 0.30 \\
$\downarrow$TER & 0.00 & \bf0.38 & 0.41 & 0.13 & 0.06 & 0.12 & 0.49 & 0.03 & 0.13 & 0.02 & 0.05 & \bf0.21 & 0.13 & 0.20 & 0.50 \\
$\uparrow$BLEU & -0.06 & -0.28 & -0.42 & -0.04 & -0.11 & -0.11 & -0.48 & -0.04 & -0.04 & \bf-0.11 & -0.06 & -0.12 & -0.10 & -0.17 & -0.48 \\
$\uparrow$METEOR & -0.10 & -0.17 & -0.32 & -0.00 & -0.17 & -0.10 & -0.38 & 0.03 & -0.00 & 0.01 & -0.02 & \bf-0.20 & 0.02 & -0.00 & -0.32 \\
$\uparrow$BERTScore & -0.01 & \bf-0.35 & \bf-0.51 & -0.09 & \bf-0.24 & \bf-0.15 & \bf-0.63 & -0.05 & -0.09 & -0.09 & -0.05 & -0.15 & -0.17 & -0.23 & \bf-0.64 \\
$\uparrow$$\conf$ & -0.04 & \bf-0.40 & \bf-0.46 & -0.16 & -0.10 & -0.10 & \bf-0.56 & -0.00 & -0.16 & \bf-0.10 & 0.09 & \bf-0.22 & 0.01 & -0.09 & -0.51 \\
%$\lx$ & 0.09 & 0.26 & 0.20 & 0.16 & 0.15 & 0.09 & 0.31 & \bf0.15 & 0.16 & 0.08 & 0.05 & -0.02 & \bf0.30 & \bf0.36 & 0.41 \\
%$\ly$ & 0.13 & 0.15 & 0.10 & 0.07 & 0.14 & 0.07 & 0.19 & 0.07 & 0.07 & 0.09 & 0.05 & -0.04 & 0.20 & 0.24 & 0.26 \\
%$\lhyp$ & 0.07 & 0.38 & 0.30 & \bf0.21 & 0.01 & 0.10 & 0.39 & 0.12 & \bf0.21 & 0.08 & 0.07 & -0.04 & \bf0.28 & \bf0.36 & 0.48 \\
%$\ratio$ & -0.04 & 0.24 & 0.22 & 0.05 & \bf-0.31 & 0.03 & 0.16 & -0.07 & 0.05 & 0.02 & 0.08 & -0.03 & -0.05 & 0.01 & 0.14 \\
\hline
\end{tabular}


==> tables/corr/pa_online_ende.tex <==
\begin{tabular}{r|rrrrrr|r|rrrrrr|r|r}
\hline
& ac & ad & mt & ne & om & ol & ac+ & fl & du & gr & ty & un & wo & fl+& ac+fl\\ 
\hline
LD &  & 0.21 & 0.04 & 0.14 & 0.13 & 0.26 & 0.23 & -0.02 & 0.14 & 0.14 & 0.10 & 0.14 & \bf0.23 & 0.25 & 0.30 \\
$\downarrow$TER &  & 0.22 & 0.05 & \bf0.17 & 0.17 & 0.18 & 0.21 & 0.02 & \bf0.17 & 0.03 & -0.01 & 0.18 & 0.04 & 0.08 & 0.18 \\
$\uparrow$BLEU &  & \bf-0.24 & -0.24 & -0.13 & \bf-0.25 & \bf-0.28 & -0.40 & -0.08 & -0.13 & -0.19 & 0.04 & -0.19 & -0.14 & -0.22 & \bf-0.39 \\
$\uparrow$METEOR &  & -0.21 & -0.21 & 0.02 & \bf-0.24 & -0.22 & -0.33 & -0.07 & 0.02 & -0.10 & 0.06 & \bf-0.23 & -0.07 & -0.11 & -0.28 \\
$\uparrow$BERTScore &  & -0.23 & -0.20 & -0.06 & \bf-0.25 & \bf-0.34 & -0.41 & -0.12 & -0.06 & -0.10 & 0.03 & \bf-0.25 & -0.17 & -0.18 & -0.38 \\
$\uparrow$$\conf$ &  & \bf-0.30 &\bf-0.56 & -0.14 & \bf-0.35 &\bf-0.27 & \bf-0.66 & -0.12 & -0.14 & \bf-0.28 & 0.00 & -0.19 & -0.18 & \bf-0.32 & \bf-0.63 \\
$\lx$ &  & 0.14 & 0.26 & 0.12 & 0.13 & \bf0.33 & 0.38 & \bf0.17 & 0.12 & \bf0.30 & 0.12 & 0.15 & \bf0.25 & \bf0.40 & \bf0.49 \\
%$\ly$ &  & 0.04 & 0.25 & -0.03 & 0.07 & 0.22 & 0.27 & \bf0.16 & -0.03 & 0.25 & 0.02 & 0.09 & 0.20 & 0.29 & 0.35 \\
$\lhyp$ &  & 0.17 & 0.22 & 0.10 & 0.05 & \bf0.33 & 0.33 & \bf0.19 & 0.10 & \bf0.26 & 0.04 & 0.16 & 0.19 & \bf0.33 & 0.41 \\
$\ratio$ &  & 0.11 & -0.08 & -0.00 & -0.17 & 0.04 & -0.06 & 0.08 & -0.00 & -0.07 & \bf-0.17 & 0.05 & -0.11 & -0.13 & -0.12 \\
\hline
\end{tabular}


==> tables/corr/tf_offline_deen.tex <==
\begin{tabular}{rrrrrrr|r|rrrrrr|r|r}
\hline
& ac & ad & mt & ne & om & ol & ac+ & fl & du & gr & ty & un & wo & fl+ & ac+fl \\ 
\hline
LD & 0.04 & 0.08 & 0.12 & 0.11 & 0.03 & -0.01 & 0.14 & -0.07 & 0.11 & -0.04 & -0.02 & 0.05 & 0.16 & 0.11 & 0.17 \\
$\downarrow$TER & -0.04 & \bf0.43 & 0.42 & 0.10 & 0.07 & 0.14 & 0.53 & 0.05 & 0.10 & 0.04 & -0.04 & \bf0.20 & 0.17 & 0.17 & 0.54 \\
$\uparrow$BLEU & 0.02 & -0.28 & -0.41 & -0.08 & -0.13 & -0.12 & -0.48 & \bf-0.10 & -0.08 & \bf-0.11 & 0.02 & -0.10 & \bf-0.19 & \bf-0.21 & -0.51 \\
$\uparrow$METEOR & 0.01 & -0.23 & -0.42 & -0.06 & -0.12 & -0.13 & -0.46 & -0.09 & -0.06 & -0.00 & 0.02 & -0.14 & -0.12 & -0.12 & -0.46 \\
$\uparrow$BERTScore & -0.02 & -0.33 & \bf-0.60 & -0.10 & -0.10 & \bf-0.15 & \bf-0.63 & -0.08 & -0.10 & -0.09 & -0.01 & -0.09 & -0.17 & \bf-0.20 & \bf-0.64 \\
$\uparrow$$\conf$ & \bf-0.13 & \bf-0.46 & \bf-0.54 & -0.04 & -0.14 & \bf-0.15 & \bf-0.66 & -0.01 & -0.04 & -0.05 & \bf0.11 & -0.14 & -0.03 & -0.02 & -0.59 \\
%$\lx$ & 0.04 & 0.02 & 0.09 & 0.17 & \bf0.20 & 0.05 & 0.14 & 0.06 & 0.17 & 0.07 & -0.01 & -0.08 & \bf0.20 & \bf0.22 & 0.21 \\
%$\ly$ & 0.07 & 0.00 & 0.05 & 0.22 & 0.14 & 0.07 & 0.09 & 0.06 & 0.22 & 0.10 & 0.03 & -0.12 & 0.11 & 0.19 & 0.16 \\
%$\lhyp$ & 0.07 & 0.20 & 0.20 & \bf0.23 & 0.10 & 0.10 & 0.27 & 0.03 & \bf0.23 & \bf0.10 & -0.00 & -0.06 & 0.15 & \bf0.22 & 0.32 \\
%$\ratio$ & 0.06 & 0.35 & 0.17 & 0.08 & \bf-0.19 & 0.09 & 0.21 & -0.09 & 0.08 & 0.05 & 0.03 & 0.03 & -0.08 & -0.01 & 0.18 \\
\hline
\end{tabular}


==> tables/corr/tf_offline_ende.tex <==
\begin{tabular}{r|rrrrrr|r|rrrrrr|r|r}
\hline
& ac & ad & mt & ne & om & ol & ac+ & fl & du & gr & ty & un & wo & fl+& ac+fl\\ 
\hline
LD &  & 0.05 & 0.02 & 0.02 & -0.09 & \bf0.20 & 0.10 & -0.01 & 0.02 & 0.18 & -0.01 & 0.08 & \bf0.25 & 0.20 & 0.19 \\
$\downarrow$TER &  & 0.18 & 0.08 & \bf0.26 & 0.11 & 0.12 & 0.20 & 0.01 & \bf0.26 & 0.01 & 0.09 & 0.15 & \bf0.25 & 0.17 & 0.24 \\
$\uparrow$BLEU &  & -0.09 & \bf-0.22 & -0.21 & \bf-0.21 & \bf-0.18 & -0.35 & -0.04 & -0.21 & -0.08 & -0.08 & -0.15 & -0.18 & -0.19 & \bf-0.35 \\
$\uparrow$METEOR &  & -0.13 & -0.19 & -0.23 & \bf-0.20 & -0.10 & -0.27 & -0.01 & -0.23 & -0.06 & -0.06 & -0.15 & -0.13 & -0.16 & -0.28 \\
$\uparrow$BERTScore &  & -0.19 & -0.18 & -0.19 & -0.16 & -0.15 & -0.32 & -0.03 & -0.19 & -0.05 & -0.05 & -0.23 & \bf-0.26 & -0.19 & -0.33 \\
$\uparrow$$\conf$ &  & \bf-0.34 & \bf-0.39 & \bf-0.27 & \bf-0.22 & -0.10 & \bf-0.51 & -0.10 & \bf-0.27 & -0.01 & -0.07 & \bf-0.33 & -0.09 & -0.16 & \bf-0.44 \\
$\lx$ &  & 0.03 & 0.12 & 0.05 & 0.15 & \bf0.20 & 0.23 & 0.08 & 0.05 & \bf0.24 & 0.07 & 0.20 & 0.11 & \bf0.27 & 0.31 \\
%$\ly$ &  & 0.03 & 0.07 & -0.01 & 0.14 & 0.14 & 0.18 & 0.09 & -0.01 & \bf0.24 & 0.09 & 0.16 & 0.03 & 0.23 & 0.26 \\
$\lhyp$ &  & 0.20 & 0.06 & 0.12 & 0.03 & \bf0.25 & 0.23 & \bf0.15 & 0.12 & \bf0.22 & \bf0.13 & \bf0.28 & 0.18 & \bf0.32 & \bf0.35 \\
$\ratio$ &  & \bf0.33 & -0.11 & 0.11 & -0.19 & 0.13 & 0.02 & \bf0.16 & 0.11 & -0.00 & \bf0.10 & 0.16 & 0.12 & 0.14 & 0.09 \\
\hline
\end{tabular}


==> tables/corr/tf_online_deen.tex <==
\begin{tabular}{rrrrrrr|r|rrrrrr|r|r}
\hline
& ac & ad & mt & ne & om & ol & ac+ & fl & du & gr & ty & un & wo & fl+ & ac+fl \\ 
\hline
LD & -0.07 & 0.26 & 0.21 & 0.16 & 0.10 & 0.05 & 0.29 & -0.01 & 0.16 & \bf-0.13 & -0.02 & -0.03 & 0.22 & 0.18 & 0.31 \\
$\downarrow$TER & 0.04 & \bf0.39 & 0.40 & \bf0.30 & 0.06 & \bf0.26 & 0.50 & -0.00 & \bf0.30 & -0.02 & 0.07 & \bf0.29 & 0.11 & \bf0.30 & \bf0.54 \\
$\uparrow$BLEU & -0.07 & -0.33 & -0.41 & \bf-0.23 & -0.11 & -0.20 & -0.48 & -0.04 & -0.23 & -0.04 & -0.08 & -0.12 & -0.09 & -0.24 & -0.50 \\
$\uparrow$METEOR & -0.08 & -0.20 & -0.42 & -0.13 & -0.08 & -0.16 & -0.41 & -0.01 & -0.13 & 0.04 & \bf-0.13 & -0.16 & -0.11 & -0.17 & -0.41 \\
$\uparrow$BERTScore & -0.09 & \bf-0.38 & \bf-0.54 & -0.21 & \bf-0.21 & \bf-0.23 & \bf-0.62 & 0.02 & -0.21 & -0.03 & -0.04 & \bf-0.28 & -0.13 & -0.24 & \bf-0.61 \\
$\conf$ & -0.11 & \bf-0.41 & \bf-0.50 & -0.21 & -0.10 & -0.20 & \bf-0.58 & 0.00 & -0.21 & \bf-0.10 & 0.04 & \bf-0.26 & -0.02 & -0.18 & \bf-0.55 \\
%$\lx$ & \bf0.14 & 0.19 & 0.12 & 0.17 & \bf0.19 & 0.08 & 0.24 & 0.08 & 0.17 & 0.04 & -0.05 & -0.14 & \bf0.33 & 0.27 & 0.32 \\
%$\ly$ & 0.14 & 0.10 & 0.10 & 0.01 & 0.14 & 0.01 & 0.15 & 0.09 & 0.01 & 0.03 & -0.02 & -0.11 & 0.22 & 0.11 & 0.17 \\
%$\lhyp$ & 0.11 & 0.32 & 0.24 & \bf0.30 & 0.11 & 0.17 & 0.36 & 0.07 & \bf0.30 & 0.04 & -0.02 & -0.05 & \bf0.30 & \bf0.36 & 0.46 \\
%$\ratio$ & -0.05 & 0.23 & 0.23 & \bf0.22 & -0.15 & 0.15 & 0.24 & -0.04 & 0.22 & 0.02 & 0.08 & \bf0.30 & -0.08 & 0.16 & 0.26 \\
\hline
\end{tabular}


==> tables/corr/tf_online_ende.tex <==
\begin{tabular}{r|rrrrrr|r|rrrrrr|r|r}
\hline
& ac & ad & mt & ne & om & ol & ac+ & fl & du & gr & ty & un & wo & fl+& ac+fl\\ 
\hline
LD & -0.00 & 0.15 & \bf0.26 & 0.02 & 0.07 & 0.09 & 0.22 & -0.03 & 0.02 & 0.07 & 0.05 & 0.14 & 0.08 & 0.10 & 0.21 \\
$\downarrow$TER & -0.00 & 0.22 & 0.22 & \bf0.25 & 0.10 & 0.11 & 0.25 & -0.07 & \bf0.25 & 0.11 & -0.00 & 0.21 & 0.19 & 0.23 & 0.30 \\
$\uparrow$BLEU & -0.06 & -0.24 & \bf-0.26 & -0.18 & -0.25 & -0.16 & -0.36 & 0.06 & -0.18 & \bf-0.19 & -0.02 & -0.21 & \bf-0.21 & -0.27 & -0.39 \\
$\uparrow$METEOR & -0.00 & -0.14 & \bf-0.27 & -0.01 & -0.24 & -0.13 & -0.32 & 0.06 & -0.01 & -0.10 & 0.03 & -0.24 & -0.15 & -0.12 & -0.28 \\
$\uparrow$BERTScore & -0.05 & -0.25 & \bf-0.31 & -0.11 & -0.24 & \bf-0.26 & \bf-0.43 & 0.08 & -0.11 & -0.08 & 0.02 & \bf-0.32 & \bf-0.20 & -0.17 & -0.38 \\
$\uparrow$$\conf$ & 0.02 & \bf-0.48 & \bf-0.44 & \bf-0.28 & \bf-0.40 & \bf-0.24 & \bf-0.66 & 0.00 & \bf-0.28 & -0.17 & -0.06 & \bf-0.26 & \bf-0.20 & \bf-0.31 & \bf-0.62 \\
$\lx$ & -0.01 & 0.29 & 0.24 & 0.17 & 0.19 & \bf0.26 & 0.34 & \bf0.12 & 0.17 & \bf0.23 & \bf0.11 & 0.14 & 0.16 & \bf0.32 & \bf0.42 \\
%$\ly$ & 0.03 & 0.11 & 0.16 & 0.02 & 0.21 & 0.18 & 0.23 & 0.10 & 0.02 & 0.17 & 0.06 & 0.10 & 0.10 & 0.19 & 0.27 \\
$\lhyp$ & 0.05 & \bf0.36 & 0.21 & \bf0.27 & 0.15 & \bf0.25 & 0.34 & \bf0.12 & \bf0.27 & \bf0.20 & \bf0.11 & 0.18 & \bf0.20 & \bf0.35 & \bf0.44 \\
$\ratio$ & 0.13 & 0.22 & -0.00 & \bf0.25 & -0.05 & 0.02 & 0.07 & 0.03 & \bf0.25 & -0.01 & 0.01 & 0.09 & 0.13 & 0.14 & 0.13 \\
\hline
\end{tabular}


==> tables/mt_length_samples.tex <==
\small
\begin{tabular}{lHp{4cm}p{4cm}p{4cm}rHrrr}
\toprule
& ID & Source & Reference & Hypothesis & \#mt & LD & $\ly$ & $|\tilde \y|$&  $\#mt/\ly$\\ 
\midrule
PA O & 114 
           & Frosty, der Kohlenmann wird jeden Tag sauberer.
           & Frosty the coal man is getting cleaner everyday. 
           & Froty, the hydrocarbons, is going to make clean every day.
           & 5 & 1.45 &   9 & 13 & 0.56 \\ 
\midrule
PA F &  97 
            & Wobei denen die Sprache untergeordnet von untergeordnetem Rang war.
            & And for them language had inferior importance. 
            & What the language was underheld by subamene-net Rang.
            & 4 & 3.78 &   8 & 11 & 0.50 \\ 
\midrule
TF F &  97 
            & Wobei denen die Sprache untergeordnet von untergeordnetem Rang war.
            & And for them language had inferior importance. 
            & What the language was signed by the bottom line. 
            & 4 & 3.78 &   8 & 10 & 0.50 \\ 
\midrule
TF O &  97 
           & Wobei denen die Sprache untergeordnet von untergeordnetem Rang war.
           & And for them language had inferior importance. 
           & What those of the language have been subordinating with is the language of subset fours.
           & 4 & 3.78 &   8 & \bad16 & 0.50 \\ 
\midrule
PA F & \bad167 
            & Ein erstaunliches Beispiel, wie eine Nation, ein Staat, die Wiedergutmachung mit seinen Einwohnern suchen und erreichen kann.
            & An amazing example of how a nation-state can seek restitution with its people. 
            & An amazing example, like a nation, a state that can look and reach rebel with their people.  
            & 6 & 3.59 &  14 & \bad20 & 0.43 \\ 
\midrule
TF F &  22 
            & In diesem unserem Land gibt es für Kinder lebenslängliche Haftstrafen ohne bedingte Strafaussetzung.
            & We have life imprisonment without parole for kids in this country. 
            & In this country, we have for children's lifetimes disruption without unconditional disagreements.  
            & 5 & 5.40 &  12 & 15 & 0.42 \\ 
\midrule
TF O &  85 
           & Aber niederlassen ist nicht immer so eine schlechte Sache.
           & But settling isn't always such a bad thing. 
           & But let's not always let it be a bad thing.
           & 4 & 0.91 &  10 & 12 & 0.40 \\ 
\midrule
TF O &  23 
           & "2.5 zu eins was? Was füttert ihr?"
           & 2.5 what? What are you feeding? 
           & "Two: Two to one thing? What do you feed?" 
           & 3 & 1.95 &   8 & 14 & 0.38 \\ 
\midrule
PA O &  37 
           & Seine Mutter wurde eingesperrt, als Bestrafung für - für das Verbrechen wohlhabend zu sein.
           & His mother was incarcerated for the crime of being wealthy. 
           & His mother was locked in when you were a punishment for - for the crime to be wealthy.  
           & 4 & 1.69 &  11 & \bad19 & 0.36 \\ 
\midrule
PA F & 196 
            & Interpreten sind Übersetzer der geschriebenen Noten in klingende Musik.
            & Interpreters are translators of the written notes in resounding music. 
            & The interpreters are the translator of the written grades in clinical music.
            & 4 & 1.07 &  11 & 13 & 0.36 \\ 
\bottomrule
\end{tabular}


==> tables/srcpostags/counts.tex <==
\begin{tabular}{rrrrrrrrrrrrrr}
\multicolumn{14}{c}{\engde}\\
\toprule
ADJ & ADP & ADV & CCONJ & DET & INTJ & NOUN & NUM & PART & PRON & PROPN & PUNCT & SYM & VERB \\
\midrule
197 & 366 & 239 & 120 & 399 &   2 & 642 &  45 & 165 & 336 &  52 & 440 &   3 & 615 \\
\bottomrule
\end{tabular}
\begin{tabular}{rrrrrrrrrrrrrrrr}
\multicolumn{16}{c}{\deen}\\
\toprule
ADJ & ADP & ADV & AUX & CCONJ & DET & INTJ & NOUN & NUM & PART & PRON & PROPN & PUNCT & SCONJ & VERB & X \\
\midrule
210 & 219 & 235 & 181 & 125 & 341 &   1 & 517 &  28 &  72 & 376 &  41 & 475 &  60 & 345 &   3 \\
\bottomrule
\end{tabular}



==> tables/srcpostags/pa_offline.tex <==
\begin{tabular}{rrrrrrrrrrrrrrr}
\toprule
& ADJ & ADP & ADV & CCONJ & DET & INTJ & NOUN & NUM & PART & PRON & PROPN & PUNCT & SYM & VERB \\
\midrule
ac& 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
ad& 0 & 2 & 5 & 0 & 2 & 0 & 4 & 1 & 1 & 3 & 0 & 2 & 0 & 3 \\ 
du& 0 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\ 
flu& 3 & 5 & 2 & 1 & 2 & 0 & 3 & 0 & 0 & 1 & 0 & 3 & 0 & 10 \\ 
gr& 14 & 38 & 5 & 2 & 19 & 0 & 22 & 4 & 7 & 10 & 1 & 5 & 0 & 36 \\ 
mt& 31 & 25 & 15 & 7 & 23 & 1 & 66 & 2 & 15 & 8 & 2 & 5 & 0 & 92 \\ 
ne& 1 & 1 & 0 & 0 & 3 & 0 & 21 & 0 & 1 & 0 & 4 & 2 & 0 & 5 \\ 
om& 6 & 23 & 11 & 4 & 13 & 0 & 19 & 0 & 10 & 6 & 1 & 10 & 0 & 27 \\ 
ol& 21 & 47 & 18 & 1 & 32 & 0 & 58 & 5 & 16 & 10 & 7 & 11 & 0 & 63 \\ 
ty& 7 & 6 & 2 & 1 & 1 & 0 & 15 & 2 & 2 & 2 & 5 & 5 & 0 & 3 \\ 
un& 2 & 4 & 2 & 1 & 2 & 0 & 6 & 0 & 3 & 1 & 1 & 3 & 0 & 6 \\ 
wo& 3 & 7 & 5 & 0 & 1 & 0 & 14 & 0 & 5 & 4 & 2 & 1 & 0 & 17 \\ 
\bottomrule
\end{tabular}


==> tables/srcpostags/pa_online.tex <==
\begin{tabular}{Hrrrrrrrrrrrrrr}
\toprule
& ADJ & ADP & ADV & CCONJ & DET & INTJ & NOUN & NUM & PART & PRON & PROPN & PUNCT & SYM & VERB \\ 
\midrule
Accuracy & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
Addition & 3 & 3 & 5 & 1 & 4 & 0 & 6 & 0 & 0 & 4 & 0 & 1 & 0 & 18 \\ 
Duplication & 0 & 3 & 1 & 0 & 2 & 0 & 6 & 0 & 2 & 4 & 0 & 3 & 0 & 4 \\ 
Fluency & 1 & 3 & 2 & 1 & 2 & 0 & 2 & 0 & 1 & 2 & 0 & 3 & 0 & 6 \\ 
Grammar & 16 & 32 & 5 & 1 & 30 & 0 & 32 & 8 & 10 & 12 & 2 & 12 & 0 & 45 \\ 
Mistranslation & 24 & 24 & 16 & 1 & 22 & 1 & 79 & 2 & 13 & 12 & 5 & 8 & 0 & 91 \\ 
NonExistingWordForm & 4 & 4 & 1 & 1 & 4 & 0 & 21 & 0 & 2 & 0 & 3 & 2 & 0 & 9 \\ 
Omission & 6 & 16 & 15 & 1 & 9 & 0 & 22 & 2 & 7 & 6 & 5 & 7 & 0 & 26 \\ 
OverlyLitteral & 29 & 63 & 19 & 1 & 42 & 0 & 67 & 5 & 18 & 13 & 8 & 14 & 0 & 69 \\ 
Typography & 5 & 3 & 2 & 2 & 2 & 0 & 19 & 3 & 2 & 3 & 4 & 9 & 1 & 8 \\ 
Unintelligible & 3 & 8 & 5 & 1 & 6 & 0 & 11 & 1 & 3 & 2 & 0 & 5 & 1 & 11 \\ 
WordOrder & 3 & 9 & 4 & 0 & 6 & 0 & 17 & 0 & 13 & 5 & 1 & 4 & 0 & 33 \\ 
\bottomrule
\end{tabular}


==> tables/srcpostags/tf_offline.tex <==
\begin{tabular}{rrrrrrrrrrrrrrr}
\toprule
& ADJ & ADP & ADV & CCONJ & DET & INTJ & NOUN & NUM & PART & PRON & PROPN & PUNCT & SYM & VERB \\ 
\midrule
ac& 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
ad& 0 & 3 & 3 & 0 & 1 & 0 & 5 & 1 & 1 & 1 & 1 & 0 & 0 & 6 \\ 
du& 1 & 3 & 2 & 0 & 0 & 0 & 3 & 0 & 1 & 3 & 1 & 0 & 0 & 4 \\ 
fl& 3 & 1 & 2 & 1 & 1 & 0 & 0 & 0 & 1 & 2 & 0 & 1 & 0 & 7 \\ 
gr& 16 & 24 & 2 & 1 & 12 & 0 & 13 & 1 & 7 & 4 & 1 & 2 & 0 & 12 \\ 
mt& 21 & 22 & 15 & 2 & 14 & 0 & 66 & 2 & 18 & 7 & 3 & 4 & 0 & 78 \\ 
ne& 2 & 0 & 2 & 2 & 4 & 0 & 18 & 1 & 0 & 1 & 1 & 3 & 0 & 2 \\ 
om& 6 & 22 & 23 & 4 & 15 & 0 & 27 & 3 & 11 & 11 & 2 & 10 & 0 & 35 \\ 
ol& 19 & 49 & 11 & 3 & 22 & 0 & 48 & 2 & 11 & 8 & 4 & 4 & 0 & 50 \\ 
ol& 3 & 3 & 3 & 1 & 1 & 0 & 8 & 3 & 1 & 2 & 7 & 4 & 0 & 2 \\ 
un& 4 & 13 & 5 & 1 & 10 & 0 & 16 & 2 & 6 & 2 & 1 & 2 & 0 & 17 \\ 
wo& 1 & 9 & 2 & 0 & 4 & 0 & 9 & 0 & 3 & 4 & 2 & 1 & 0 & 16 \\ 
\bottomrule
\end{tabular}


==> tables/srcpostags/tf_online.tex <==
\begin{tabular}{Hrrrrrrrrrrrrrr}
\toprule
& ADJ & ADP & ADV & CCONJ & DET & INTJ & NOUN & NUM & PART & PRON & PROPN & PUNCT & SYM & VERB \\ 
\midrule
Accuracy & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 
Addition & 4 & 7 & 3 & 0 & 6 & 0 & 6 & 0 & 2 & 6 & 0 & 7 & 0 & 13 \\ 
Duplication & 5 & 9 & 7 & 3 & 9 & 0 & 18 & 2 & 4 & 9 & 1 & 5 & 0 & 19 \\ 
Fluency & 3 & 3 & 2 & 1 & 2 & 0 & 5 & 0 & 0 & 0 & 0 & 3 & 0 & 7 \\ 
Grammar & 13 & 24 & 4 & 1 & 34 & 0 & 18 & 5 & 10 & 8 & 1 & 3 & 0 & 24 \\ 
Mistranslation & 27 & 32 & 14 & 3 & 19 & 1 & 74 & 1 & 18 & 10 & 6 & 5 & 1 & 88 \\ 
NonExistingWordForm & 7 & 2 & 0 & 1 & 5 & 0 & 22 & 0 & 1 & 0 & 2 & 1 & 0 & 5 \\ 
Omission & 7 & 22 & 10 & 1 & 9 & 0 & 34 & 3 & 8 & 6 & 0 & 6 & 0 & 32 \\ 
OverlyLitteral & 17 & 43 & 17 & 1 & 25 & 0 & 55 & 2 & 15 & 15 & 3 & 9 & 0 & 58 \\ 
Typography & 8 & 3 & 4 & 2 & 1 & 0 & 12 & 2 & 2 & 2 & 4 & 10 & 0 & 6 \\ 
Unintelligible & 5 & 14 & 6 & 1 & 12 & 0 & 15 & 1 & 6 & 4 & 0 & 4 & 0 & 21 \\ 
WordOrder & 6 & 13 & 5 & 0 & 8 & 0 & 13 & 1 & 9 & 4 & 1 & 4 & 0 & 30 \\ 
\bottomrule
\end{tabular}


==> tables/whos_the_winner.tex <==
\begin{tabular}{lcccccccccc}
\toprule
 &  BLEU  &  METEOR  &  ROUGE-L  &  RIBES  &   BLEU  &  METEOR  &  ROUGE-L  &  RIBES  &  \#accuracy  &  \#fluency \\
\midrule
De$\sto$En offline & PA & PA & TF & TF & PA & PA & PA(+0.03) & TF & PA & TF\\
De$\sto$En online  & PA & TF & TF & PA & TF & TF & TF & TF & PA(+3) & PA\\
\midrule
En$\sto$De offline & TF & TF & TF(+0.05) & TF & TF & TF(+0.03) & TF & TF & TF & TF\\
En$\sto$De online  & PA(+0.05) & TF & TF & PA & PA & TF & PA & PA & PA & TF(+1)\\
\bottomrule
\end{tabular}

